Revisiting Temporal Blocking Stencil Optimizations

Iterative stencils are used widely across the spectrum of High Performance Computing (HPC) applications. Many efforts have been put into optimizing stencil GPU kernels, given the prevalence of GPU-accelerated supercomputers. To improve the data locality, temporal blocking is an optimization that combines a batch of time steps to process them together. Under the observation that GPUs are evolving to resemble CPUs in some aspects, we revisit temporal blocking optimizations for GPUs. We explore how temporal blocking schemes can be adapted to the new features in the recent Nvidia GPUs, including large scratchpad memory, hardware prefetching, and device-wide synchronization. We propose a novel temporal blocking method, EBISU, which champions low device occupancy to drive aggressive deep temporal blocking on large tiles that are executed tile-by-tile. We compare EBISU with state-of-the-art temporal blocking libraries: STENCILGEN and AN5D. We also compare with state-of-the-art stencil auto-tuning tools that are equipped with temporal blocking optimizations: ARTEMIS and DRSTENCIL. Over a wide range of stencil benchmarks, EBISU achieves speedups up to $2.53$x and a geometric mean speedup of $1.49$x over the best state-of-the-art performance in each stencil benchmark.

==> 07_03_discussion.tex <==
\revision{
\subsection{Discussion}
% \subsection{General GPU Optimizations}
% This paper we shows that changing perspective of GPU optimization from constraining resources for parallelism to constraining parallelism for resources can benefit a sufficiently studied computing pattern, stencils.  2x speedup over SoTA libraries for a wide range of stencil benchmarks. That is despite the fact that SoTA libraries have been optimized and tuned at the fine-grained instruction level to avoid pressure on resources. We hope that EBISU would not just be of value for stencil research, but also open venues for researchers using GPUs in HPC in general to revisit GPU optimization approaches with consideration of how GPUs have evolved
%As such, additional research and engineering are necessary to push EBISU for practical applications.
% This paper focuses on studying how modern GPU characteristics influence the optimization of temporal blocking stencils. 
% \subsection{Practical EBISU}
% \subsubsection{Automatically Adjust }
% This paper focuses on studying how modern GPU characteristics influence the optimization of temporal blocking stencils. Nevertheless, as EBISU proved effective, its optimization approach can be absorbed into production libraries like Halide~\cite{ragan2013halide} so that the end user can get the performance with minimal effort.
% We acknowledged, that there are still consideration that we haven't explored. Examples include load balance when applying one tile at a tile, and different combinations of thread, thread block and grid tiling. 


}

==> 09_discussion.tex <==
\revision{
\section{Discussion and Future Works}
\subsection{General GPU Optimizations}
This paper we shows that changing perspective of GPU optimization from constraining resources for parallelism to constraining parallelism for resources can benefit a sufficiently studied computing pattern, stencils.  2x speedup over SoTA libraries for a wide range of stencil benchmarks. That is despite the fact that SoTA libraries have been optimized and tuned at the fine-grained instruction level to avoid pressure on resources. We hope that EBISU would not just be of value for stencil research, but also open venues for researchers using GPUs in HPC in general to revisit GPU optimization approaches with consideration of how GPUs have evolved

\subsection{Practical EBISU}
% \subsubsection{Automatically Adjust }
We consider this research a pioneering research. We acknowledged, that there are still consideration that we haven't explored. Examples include load balance when applying one tile at a tile, different combinations of thread, thread block and grid tiling, and combinations of optimizations as well as adding existing optimizations. As such, additional research and engineering are necessary to push EBISU for practical applications.

% This paper focuses on studying how modern GPU characteristics influence the optimization of temporal blocking stencils. 
Nevertheless, as EBISU proved effective, its optimization approach can be absorbed into production libraries like Halide~\cite{ragan2013halide} so that the end user can get the performance with minimal effort.

\subsection{On-chip Resources Management}
We in this study explored A100 that equipped with sufficient large L1 cache (164 KB scratchpad memory). So we don't need to manage the on-chip resources. However, when it comes a general cases, we interested in how much performance degrade EBISU might suffer if port it to any existing architecture with more restricted shared memory capacity, e.g. 64 KB in MI250 and 96 KB in V100. And how much performance benefit we might gain with next generation architecture with larger cache, e.g. 228 KB in H100. 

\subsection{White Box Performance Model}
This research shows a potential of using white box performance model to support implementation decisions. The correct analysis of applying grid tile enhance performance decision. However, grid level synchronization is easier to model than thread block level synchronization. We are also working on a extension of performance model for a even more accurate implementation decisions. 

% We also interested in  

%Though we can also waiting all architectures to cache up the capacity of L1 cache, a study of EBISU in the environment of restricted cache capacity is necessary to push EBISU to a wider . 

% we should extend EBISU to general cases when on-chip resources become restricted. 
% However, when the cache become restricted, a better management of resources would be necessary. 

% \subsection{EBISU for End-Users}

% \todo{The experimental results are not explained well. The evaluation section is too short and provides little discussion. For example, in Figure 8, the reviewer noticed that for some benchmarks, EBISU has even higher register utilization, which is contrary to Section 8.3’s claim. This needs more discussion.}
}


==> LISTING/2_5_D_temporal_blocking_2d5pt.tex <==

\lstset{
 	language = C++, breaklines = true, breakindent = 10pt, lineskip={-1pt}, basicstyle = \rmfamily\scriptsize, commentstyle = {\itshape \color[cmyk]{1,0.4,1,0}}, classoffset = 0, keywordstyle = {\bfseries \color[cmyk]{0,1,0,0}}, stringstyle = {\ttfamily \color[rgb]{0,0,1}}, frame = trbl, framesep=0pt, numbers = left, stepnumber = 1, xrightmargin=12pt, xleftmargin=0pt, numberstyle = \tiny, tabsize = 1, captionpos = t, directivestyle={\color{black}},  emph={int,char,double,float,unsigned, int3, float4, float2}, emphstyle={\color{blue}},
}
\lstset{escapeinside={<@}{@>}}

\begin{figure}[t]
\centering
\begin{minipage}[c]{0.5\textwidth}
% \footnotesize
\begin{lstlisting}[caption = {Pseudo code for 2D 5-point Jacobian Stencil, low occupancy temporal blocking, assuming using only one thread block.}, label = Fig:basictemporal]
void __global__ void 2_5D_2d5pt(...){
...
for(int tile=0; tile<total_tile; tile++)
{
    preload(input[tile][][],sm[step][][]);
    //preload represent using asynchronous copy to shared memory
    fetch(sm[step-1][][],reg[step-1][][]);
    //put part of data to register 
    for(int s=2; s<=step; s--)
    {
        2d5pt(sm[s-1][][],ref[s-1][],sm[s-2][][]);
    }
    2d5pt(sm[0][][],sm[0][][],output[loc_to_store][][]);
    __syncthreads();
    //only need to synchronize once
    shift(reg);
    shift(sm);
}
...
}
__device__ void 2d5pt(sm_in,reg_in,sm_out)
{
    for(int i=0; i<ilp i++)
    {
        sm_out[i][tid]=
            Center * ref_in[i]   +
            South  * ref_in[i-1] +
            North  * ref_in[i+1] +
            East   * sm_in[i][tid+1] +
            West   * sm_in[i][tid-1];
    }
}
\end{lstlisting}
\end{minipage}
\end{figure}


==> LISTING/grid_level_2_5_D_temporal_blocking.tex <==

\lstset{
 	language = C++, breaklines = true, breakindent = 10pt, lineskip={-1pt}, basicstyle = \rmfamily\scriptsize, commentstyle = {\itshape \color[cmyk]{1,0.4,1,0}}, classoffset = 0, keywordstyle = {\bfseries \color[cmyk]{0,1,0,0}}, stringstyle = {\ttfamily \color[rgb]{0,0,1}}, frame = trbl, framesep=0pt, numbers = left, stepnumber = 1, xrightmargin=12pt, xleftmargin=0pt, numberstyle = \tiny, tabsize = 1, captionpos = t, directivestyle={\color{black}},  emph={int,char,double,float,unsigned, int3, float4, float2}, emphstyle={\color{blue}},
}
\lstset{escapeinside={<@}{@>}}

\begin{figure}[t]
\centering
\begin{minipage}[c]{0.5\textwidth}
% \footnotesize
\begin{lstlisting}[caption = {Pseudo code for 2D 5-point Jacobian Stencil, low occupancy temporal blocking, assuming using only one thread block.}, label = Fig:grid2_5D, rulecolor=\color{blue}]
void __global__ void 3_5D_3d7pt(...){
...
for(int tile=0; tile<total_tile; tile++)
{
    preload(input[tile][][],sm[step][][]);
    preload_halo(gm_halo,sm[][][]);
    //preload represent using asynchronous copy to shared memory
    
    for(int s=2; s<=step; s--)
    {
        fetch(sm[s-1][][],reg[s-1][][]);
        //put part of data to register ()
        3d7pt(sm[s-1][][],ref[s-1][],sm[s-2][][]);
    }
    fetch(sm[0][][],reg[0][][]);
    3d7pt(sm[0][][],ref[0][],output[loc_to_store][][]);
    __syncthreads();
    store_halo(sm[][][],gm_halo);
    grid.sync();
    shift(reg);
    shift(sm);
}
...
}
\end{lstlisting}
\end{minipage}
\end{figure}


==> REBUTTAL/ICS23.tex <==
We thank all reviewers. If accepted, the final manuscript will reflect all comments.

First, we would like to emphasize that EBISU is pioneering the revisit of the basic principles that drove temporal blocking on GPUs for the last 15 years. Existing SoTA on temporal blocking constrain themselves to resource usage in a way that reflects the need for high concurrency and over-subscription. Unlike existing approaches, we do not constrain ourselves to resource usage patterns that chase high parallelism. This change in viewing how to program modern GPUs enables EBISU to achieve a 2x speedup over SoTA libraries for a wide range of stencil benchmarks. That is despite the fact that SoTA libraries have been optimized and tuned at the fine-grained instruction level to avoid pressure on resources. 
We hope that EBISU would not just be of value for stencil research, but also open venues for researchers using GPUs in HPC in general to revisit GPU optimization approaches with consideration of how GPUs have evolved (as we discuss in the paper Sections 3 and 4). 




**Q-** What applications benefit from EBISU? (Reviewer-A)
**A-** EBISU targets iterative stencils, a foundational compute pattern in numerous HPC applications (occupying up to 50\% of cycles in many HPC centers [19]). Any advance in stencil optimization benefits a wide span of HPC applications. 

**Q** How much effort it takes to apply EBISU? (Reviewer-B)
**A** This paper focuses on studying how modern GPU characteristics influence the optimization of temporal blocking stencils. However, as EBISU proved effective, its optimization approach can be absorbed into production libraries like Halide so that the end user can get the performance with minimal effort. 

**Q** How is the depth of temporal blocking determined, and how does it influence resource usage? (Reviewer B, C)
**A** The cost model (Sections 6-7) can identify the maximum depth before performance drops (due to the usage of resources that can be a bottleneck). For 2D stencils, as discussed in Section 7.2.1, we can use the cost model to find a threshold. However, the optimal depth in practice is usually slightly deeper because the model assumes a perfect memory access pattern. For 3D stencils, as indicated in Section 7.2.2, we use the deepest temporal blocking the on-chip resources can support per our cost model.

**Q** Effect of different optimizations? (Reviewer C, D)
**A** Due to space limitations, we did not include a breakdown of the performance of different optimizations in the manuscript. Should the paper be accepted, we commit to adding a case study from 2D stencils (2d5pt) and another from 3D stencils (3d7pt) to show how different optimizations contribute to the overall performance improvement.

**Q** Explanations are not clear in many places. (Reviewer-C, D)
**A** We acknowledge the issue. Should the paper be accepted, we commit to improving the explanations in the paper. Namely, we simplify Figure 6 by removing registers mapping, and we commit to restructuring Sections 6 and 7: Section 6 would discuss the performance analysis and all the implementation decisions move to Section 7. 




==> TABLE/KernelOverhead.tex <==
\begin{table}[t]
    \centering
    \caption{Overhead of a kernel (A100)}
    % \resizebox{\linewidth}{!}
    {\footnotesize
    \begin{tabular}{?c?c?c?}\tbhline
                              &\textbf{Kernel Launch}     &\textbf{Grid Sync (256x108)}  \\\hline
\textbf{Runtime (us)}         &2.2&1.2\\\hline
    \end{tabular}
    \label{tab:overhead}
    }
\end{table}


==> TABLE/ParamaterUsed.tex <==
\begin{table}[t]
    \centering
    \caption{Summary of expressions used in this paper}% SM is Steam Multiprocessor}
    % \resizebox{\linewidth}{!}
    {\footnotesize
    \begin{tabular}{?c?c?}\tbhline
\textbf{Name}            &\textbf{Explanation}\\\hline
% $TLP$                           &Thread Level Parallelism\\
% $ILP$                           &Instruction Level Parallelism\\
% $IPT$                           &Item processed Per Thread\\\hline
$rad$                           &Stencil order\\
$t$                             & Depth of temporal blocking\\
$tile_x$                        &Thread block spatial blocking, tiling width in x axle\\
$tile_y$                        &Thread block spatial blocking, tiling width in y axle\\\hline
$\mathbb{S}_{Cell}$           &Size of a cell\\
$\mathbb{S}_{SM}$             &Size of shared memory requested\\
$\mathbb{A}_{mem}$            &Total memory access times of mem in domain of interest\\
$\mathbb{A}_{cmp}$            &Total FLOPS in domain of interest\\
$\mathbb{D}_{mem}$            &Amount of cells in domain of interest for mem\\
$\mathbb{D}_{cmp}$            &Amount of cells in domain of interest for computation \\
$\mathbb{B}_{mem}$            &Memory bandwidth of mem\\
$\mathbb{THR}_{cmp}$          &Total FLOPS of the computation\\
${a}_{mem}$            &Memory access times per cell of mem\\
${a}_{cmp}$            &FLOPS per cell\\
$_{sm}$                       &Shared memory\\
$_{gm}$                       &Global memory\\\hline
$\mathbb{V}$                  &Valid proportion\\
$\mathbb{T}_c$                &Runtime of component c\\
$\mathbb{P}$                  &Attainable performance\\
% $_{gm}$            &Global Memory\\
\hline

    \end{tabular}
    \label{tab:explanations}
    }
\end{table}


==> TABLE/features2dstencil.tex <==
\begin{table}[t]
    \centering
    \caption{Summary of features for 2d stencils}% SM is Steam Multiprocessor}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{?c?c?c?c?c?}\tbhline
                              &\multicolumn{2}{c?}{\textbf{StencilGen~\cite{rawat2018domain}}}&\textbf{AN5D~\cite{DBLP:conf/cgo/MatsumuraZWEM20}}     &\textbf{This work}  \\\hline
                              &Star&Box&*&*\\\hline
\textbf{SM Access}            &{\footnotesize$4\times rad+1$}& {\footnotesize$(2\times rad+1)^2+1$}&{\footnotesize$2\times rad+1$}&{\footnotesize$2\times rad+1$}\\\hline
\textbf{Register Bound}      &\multicolumn{2}{c?}{64}&$\leq96$ & $256$\\\hline
\textbf{Sync per plane}      &\multicolumn{2}{c?}{$t$ }&$ t$ &$1$\\\hline
    \end{tabular}
    \label{tab:featurescmp}
    }
\end{table}


==> TABLE/gpu_specs.tex <==

\begin{table*}[t]
    \centering
    % \tiny
    \caption{Specifications of the graphical processing units (GPUs) for a workstation in last decades. Some from public documents and published research (marked as cite notation in the number), some collected by manually using microbenchmarks\cite{zhang2020study,wong2010demystifying,mei2016dissecting} (marked by underline)}
    \resizebox{\textwidth}{!}
    {%
    \begin{threeparttable}
    \begin{tabular}{|l|cccccc|cccc|cccc|cc|}\hline
    &&&&\multicolumn{2}{c}{{CUDA Cores/SMX}}&&\multicolumn{4}{c|}{{DFMA}}&\multicolumn{4}{c|}{{FFMA}}&\multicolumn{2}{c|}{{Peak Performance}}\\
    GPU model               & Year  & Arch   & SMX &FP64&FP32& Warps/SMX~\cite{nvidiaoccupancy}&Throughput~\cite{nvidia2019programming}&Latency~\cite{wong2010demystifying}&C&Min Occupancy~\tnote{a}&Throughput~\cite{nvidia2019programming}&Latency~\cite{wong2010demystifying}&C&Min Occupancy& Double    &Single \\
                            &       &        &  &&&&(op/cycle)&(cycle)&(op)&    & (op/cycle)&(cycle)&(op) &  & (TFLOPS/s)     &  (TFLOPS/s) \\\hline
    \multicolumn{17}{|c|}{{Tesla/ Data Center GPUs}}   \\\hline            
    Nvidia Tesla K20~\cite{kepler}                              &2013   &3.50          & $15$    &64&192   &64 &$64$     &  $\mathbf{10}$                          &  $640$    & $31.25\%$&$192$                & $\mathbf{9}$                              & $1728$    &  $84.375\%$   &$1.17$       &$3.52$\\\hline
    Nvidia Tesla P100-PCIE~\cite{nvidia2017v100,amperewhite}    &2016   &6.00          & $56$    &32&64    &64 &$32$     &  $8$~\cite{jia2018dissecting}           &  $256$    &$12.5\%$ &$64$                 & $6$~\cite{jia2018dissecting}              &$384$      &  $18.75\%$    &$5.3$        &$10.6$\\\hline
    Nvidia Tesla V100-SMX~\cite{nvidia2017v100,amperewhite}     &2017   &7.00          & $80$    &32&64    &64 &$32$     &  $8$~\cite{jia2018dissecting}           &  $256$    & $12.5\%$ &$64$                 & $4$~\cite{jia2018dissecting}              &$256$      &   $12.5\%$    &$7.8$        &$15.4$\\\hline
    Nvidia A100-PCIE~\cite{amperewhite}                         &2020   &8.00          & $108$   &32&64    & 64&$32$     &  $4$~\cite{abdelkhalik2022demystifying} & $128$     &  $6.25\%$&$64$        &$2$~\cite{abdelkhalik2022demystifying}     &$128$      &  $6.25\%$    &$9.7$        &$19.5$\\\hline
    Nvidia H100-PCIE~\cite{nvidiah100}                          &TBC    &9.00          & $114$   &32&64    &- &$64$     & -                                       &  -        &- &$128$               &-                                          &-          &  -   &$24$     &$48$  \\\hline
    Nvidia H100-SMX~\cite{nvidiah100}                           &TBC    &9.00          & $132$   &32&64    &- &$64$     & -                                       &  -        &- &$128$               &-                                          &-          &  -   &$30$     &$60$\\\hline
    \multicolumn{17}{|c|}{{Workstation/ Consumer GPUs}}   \\\hline     
    GTX 980TI~\cite{gtx980,Techpower}                           &2015   &5.20           &$22$   & -&128    &64 &$4$      &   $\mathbf{47}$                         & $188$     & $9.375\%$&$128$                &$\mathbf{6}$                               &$768$      &   $37.5\%$  &$0.189$&         $6.06$ \\\hline
    GTX 1080TI~\cite{gtx1080,turing,Techpower}                  &2017   &6.10           &$28$   & -&128    & 64&$4$      &   $\mathbf{47}$                         &  $188$    & $9.375\%$&$128$                &$\mathbf{6}$                               &$768$      &   $37.5\%$  &$0.354$&         $11.3$\\\hline
    RTX 2080TI~\cite{turing,Techpower}                          &2018   &7.50           &$68$   & -&64     & 32&$2$      &   $\mathbf{47}$                         &  $94$     &$12.5\%$ &$64 $        &$\mathbf{4}$                               &$256$      &   $25\%$  &$0.420$&         $14.2$ \\\hline
    GTX 3090 ~\cite{a102,Techpower}                             &2020   &8.60           &$82$   & - &128   &48 &$2$      &   $\mathbf{47}$                         &  $94$     &$8.33\%$ &$128$        &$\mathbf{4}$                               &$512$      &   $33.33\%$  &$0.556$&         $35.6$   \\\hline
    \end{tabular}
    \
    \begin{tabular}{|l|ccccc|cccc|ccccc|}\hline
    &\multicolumn{5}{c|}{{Shared Memory/SMX}}&\multicolumn{4}{c|}{L2 Cache}&\multicolumn{5}{c|}{{Global Memory}}\\
    GPU model               &(max)Size   &Bandwidth\cite{nvidia2019programming}      &Latency~\cite{wong2010demystifying}    &C & Min Occupancy   & Size  &Bandwidth      &Latency  &C/SMX    & Size       &Bandwidth      &Latency~\cite{zhang2022persistent}    &C/SMX & Min Occupancy    \\
                                &(KB)           &(B/clk)                                    &(cycle)    &       (B)         & (8B per access) & (MB)&   (GB/s) &(ns) &(B)& (GB)       &(GB/s)         &      (ns)   &        (B) &  (8B per access)  \\\hline
    \multicolumn{15}{|c|}{{Tesla/ Data Center GPUs}}   \\\hline            

    Nvidia Tesla K20~\cite{kepler}                              &$48$                 &       $256$ &       $\mathbf{47}$                   &$12032$&$73.44\%$  & $1.5$   &$\mathbf{287.69}$              &  $\mathbf{314.23}$  & $\mathbf{6026.72191}$  &$5$          &$208$            &     $\mathbf{480.80}$      &      6667 &    $42.19\%$    \\\hline
    Nvidia Tesla P100-PCIE~\cite{nvidia2017v100,amperewhite}    &$64$                 &       $128$ &       $24$~\cite{jia2018dissecting}   &$3072$ & $18.75\%$ & $4$ &$\mathbf{1540.09}$             &  $\mathbf{197.37}$ ($234$ cycle~\cite{jia2018dissecting})   &  $\mathbf{5459.71}$  &$12$         &$720$            & 4943         &        $\mathbf{384.49}$      &$31.25\%$   \\\hline
    Nvidia Tesla V100-SMX~\cite{nvidia2017v100,amperewhite}     &$96$                 &       $128$ &       $19$~\cite{jia2018dissecting}   &$2432$ &$15.63\%$  & $6$ &$\mathbf{2231.78}$ ($2048$bytes/clk)       &   $\mathbf{144.79}$ ($192$ cycle~\cite{jia2018dissecting})  &$\mathbf{4039.24}$&$16$         &$900$            &     $\mathbf{288.12}$      &     3241         &$20.31\%$ \\\hline
    Nvidia A100-PCIE~\cite{amperewhite}                         &$164$                &       $128$ &       $23/19$~\tnote{b}~\cite{abdelkhalik2022demystifying}       &   $2944/2432$~\tnote{b}         &$15.63\%/18.75\%$~\tnote{b}   & $40$    &$\mathbf{2543.62}$ ($5120$bytes/clk)           &  $\mathbf{144.88/314.26}$~\tnote{c} ($\mathbf{218/384}$ cycle) &$10335/18204$&$40$         &$1555$           &       $\mathbf{407.97}$    &       5874   &  $35.93\%$    \\\hline
    Nvidia H100-PCIE~\cite{nvidiah100}                          &$228$                &       $128$ &       -       &       - &-      & $50$        &-          &-    & - &$80$         &$2000$           &   -       &        - &-     \\\hline
    Nvidia H100-SMX~\cite{nvidiah100}                           &$228$                &       $128$ &       -       &       - &-      & $50$        &-          &-&-&$80$         &$3000$           &      -    &        -     &-\\\hline
    \multicolumn{15}{|c|}{{Workstation/ Consumer GPUs}}   \\\hline  
    GTX 980TI~\cite{gtx980,Techpower}                           &  $96$               &       $128$ &       $\mathbf{35}$      &       $4480$    &  $28.13\%$  & $3$        &     $\mathbf{748.15}$       &   $\mathbf{174.04}$      &   $\mathbf{5918.54}$    &$6$          &$336.6$   &  $\mathbf{299.20}$           &4578&$28.125\%$ \\\hline
    GTX 1080TI~\cite{gtx1080,turing,Techpower}                  &  $96$               &       $128$ &       $\mathbf{35}$      &       $4480$     & $28.13\%$   & $2.75$    &    $\mathbf{1204.59}$        &   $\mathbf{130.15}$     &    $\mathbf{5599.19}$   &$11$         &$484$   &    $\mathbf{235.38}$           &4068&$25\%$ \\\hline
    RTX 2080TI~\cite{turing,Techpower}                          &  $64$               &       $128$ &       $\mathbf{29}$      &       $3712$    &  $46.88\%$   & $5.5$     &   $\mathbf{1876.69}$         &    $\mathbf{111.80}$    &     $\mathbf{3085.50}$  &$11$         &$616$        &   $\mathbf{239.82}$       &2172&$28.125\%$ \\\hline
    GTX 3090~\cite{a102,Techpower}                              &  $96$               &       $128$ &       $\mathbf{29}$      &       $3712$    &  $31.25\%$   & $6$       &   $\mathbf{2041.82}$         &    $\mathbf{129.50}$   &     $\mathbf{3224.58}$  &$24$         &$936$        &   $\mathbf{267.45}$       &3052&$25\%$ \\\hline
    \end{tabular}
    \
    \begin{tabular}{|l|cc|cc|ccc|}\hline
    &\multicolumn{2}{c|}{{Shuffle}}&\multicolumn{2}{c|}{syncthreads}&\multicolumn{3}{c|}{{Latency of grid sync~\cite{zhang2020study}}}\\
    GPU model   &Throughput~\cite{nvidia2019programming}    & Latency~\cite{wong2010demystifying,zhang2020study}    &Throughput~\cite{nvidia2019programming}    & Latency~\cite{wong2010demystifying,zhang2020study}  &   &  &(max)    \\
    Block/SMX     &-    & -  &-& -    & $1$~\tnote{d}  & $\leq2$~\tnote{e}  &$32$    \\
    Thread/Block  &-    & -  &-& -   & $256$&  $\forall$ &  $64$)    \\
                &(op/clk)           &(clk)                               &(op/clk)           &(clk)                      & us & us                  & us     \\\hline
    \multicolumn{8}{|c|}{{Tesla/ Data Center GPUs}}   \\\hline            

    (kiev2 GPU0)Nvidia Tesla K20~\cite{kepler}                              &$32$ &$\mathbf{9}$                             &$128$  &$\mathbf{80}$                  &-&- &-              \\\hline
    (kiev6)Nvidia Tesla P100-PCIE~\cite{nvidia2017v100,amperewhite}         &$32$ &$31$~\cite{zhang2020study}   &$32$   & $\mathbf{138}$                &$1.83$~\cite{zhang2020study}& $1.77\sim3.52$~\cite{zhang2020study}&$28.42$~\cite{zhang2020study}   \\\hline
    (rwbc)Nvidia Tesla V100-SMX~\cite{nvidia2017v100,amperewhite}           &$32$ &$22$~\cite{zhang2020study}   &$16$   &$22$~\cite{zhang2020study}     &$1.50$~\cite{zhang2020study}&$1.43\sim3.49$~\cite{zhang2020study}&$24.51$~\cite{zhang2020study}       \\\hline
    (kiev0)Nvidia A100-PCIE~\cite{amperewhite}                              &$32$ &$\mathbf{26}$                &$16$   &$\mathbf{23}$                  &$\mathbf{1.21}$&$\mathbf{1.20\sim1.28}$& $\mathbf{18.02}$            \\\hline
    Nvidia H100-PCIE~\cite{nvidiah100}                                      &$32$ &-                            &-      &-                              &- &-&-       \\\hline
    Nvidia H100-SMX~\cite{nvidiah100}                                       &$32$ &-                            &-      &-                              &- &-&-     \\\hline
    \multicolumn{8}{|c|}{{Workstation/ Consumer GPUs}}   \\\hline  
    (kiev5)GTX 980TI~\cite{gtx980,Techpower}                                &$32$ &  $\mathbf{6}$                           &$64$   &$\mathbf{134}$&-&-&-  \\\hline
    (kiev1)GTX 1080TI~\cite{gtx1080,turing,Techpower}                       &$32$ &  $\mathbf{6}$                           &$64$   &$\mathbf{138}$&$\mathbf{1.06}$&$\mathbf{1.05\sim1.35}$&  $\mathbf{12.27}$ \\\hline
    (kiev2 GPU1)RTX 2080TI~\cite{turing,Techpower}                          &$16$ &  $\mathbf{4}$                           &$16$   &$\mathbf{22} $&$\mathbf{0.91}$&$\mathbf{0.86\sim1.57}$&  $\mathbf{5.07}$ (blk/SMX=16) \\\hline
    (roma7 GPU2)GTX 3090~\cite{a102,Techpower}                              &$32$ & $\mathbf{4}$                          &$16$   &$\mathbf{22} $&$\mathbf{0.63}$&$\mathbf{0.62\sim0.65}$&  $\mathbf{4.32}$ (blk/SMX=16) \\\hline
    \end{tabular}
    \begin{tablenotes}
    \item[a] Min occupancy is calculated by counting necessary warps to full fill concurrency (assuming thread level parallelism is the only means providing concurrency), divide it by the maximal active warps per stream multiprocessor. 
    \item[b] Load 23 cycle; Store 19 cycle.
    \item[c] We observed a clear near difference in latency between close hit and far hit. We are not sure how to use the full bandwidth of both slice of L2 cache.
    \item[d] The following research use this parameter setting. This research assume that it is possible to saturate the device with 256 threads per stream multi-processor.
    \item[e] The setting recommended by Zhang et al.~\cite{zhang2020study}.
    \end{tablenotes}
    \end{threeparttable}
    }
    \label{tab:stencil_speedups}
    % ~\tablefootnote{load 23 cycle; store 19 cycle}
\end{table*}


==> TABLE/gpuspecs.tex <==

\begin{table*}[t]
    \centering
    % \tiny
    \caption{Specifications of the graphical processing units (GPUs) for workstation in last decades. Some from public documents and published researches (marked as cite notation aside the number), some collected by manually microbenchmarks\cite{zhang2020study,wong2010demystifying,mei2016dissecting} (marked by underline)}
    \resizebox{\textwidth}{!}
    {%
    \begin{threeparttable}
    \begin{tabular}{|l|cccccc|cccc|cccc|cc|}\hline
    &&&&\multicolumn{2}{c}{{CUDA Cores/SMX}}&&\multicolumn{4}{c|}{{DFMA}}&\multicolumn{4}{c|}{{FFMA}}&\multicolumn{2}{c|}{{Peak Performance}}\\
    GPU model               & Year  & Arch   & SMX &FP64&FP32& Warps/SMX~\cite{nvidiaoccupancy}&Throughput~\cite{nvidia2019programming}&Latency~\cite{wong2010demystifying}&C&Min Occupancy~\tnote{a}&Throughput~\cite{nvidia2019programming}&Latency~\cite{wong2010demystifying}&C&Min Occupancy& Double    &Single \\
                            &       &        &  &&&&(op/cycle)&(cycle)&(op)&    & (op/cycle)&(cycle)&(op) &  & (TFLOPS/s)     &  (TFLOPS/s) \\\hline
    \multicolumn{17}{|c|}{{Tesla/ Data Center GPUs}}   \\\hline            
    Nvidia Tesla K20~\cite{kepler}                              &2013   &3.50          & $15$    &64&192   &64 &$64$     &  $\mathbf{10}$                          &  $640$    & $31.25\%$&$192$                & $\mathbf{9}$                              & $1728$    &  $84.375\%$   &$1.17$       &$3.52$\\\hline
    Nvidia Tesla P100-PCIE~\cite{nvidia2017v100,amperewhite}    &2016   &6.00          & $56$    &32&64    &64 &$32$     &  $8$~\cite{jia2018dissecting}           &  $256$    &$12.5\%$ &$64$                 & $6$~\cite{jia2018dissecting}              &$384$      &  $18.75\%$    &$5.3$        &$10.6$\\\hline
    Nvidia Tesla V100-SMX~\cite{nvidia2017v100,amperewhite}     &2017   &7.00          & $80$    &32&64    &64 &$32$     &  $8$~\cite{jia2018dissecting}           &  $256$    & $12.5\%$ &$64$                 & $4$~\cite{jia2018dissecting}              &$256$      &   $12.5\%$    &$7.8$        &$15.4$\\\hline
    Nvidia A100-PCIE~\cite{amperewhite}                         &2020   &8.00          & $108$   &32&64    & 64&$32$     &  $4$~\cite{abdelkhalik2022demystifying} & $128$     &  $6.25\%$&$64$        &$2$~\cite{abdelkhalik2022demystifying}     &$128$      &  $6.25\%$    &$9.7$        &$19.5$\\\hline
    Nvidia H100-PCIE~\cite{nvidiah100}                          &TBC    &9.00          & $114$   &32&64    &- &$64$     & -                                       &  -        &- &$128$               &-                                          &-          &  -   &$24$     &$48$  \\\hline
    Nvidia H100-SMX~\cite{nvidiah100}                           &TBC    &9.00          & $132$   &32&64    &- &$64$     & -                                       &  -        &- &$128$               &-                                          &-          &  -   &$30$     &$60$\\\hline
    \multicolumn{17}{|c|}{{Workstation/ Consumer GPUs}}   \\\hline     
    GTX 980TI~\cite{gtx980,Techpower}                           &2015   &5.20           &$22$   & -&128    &64 &$4$      &   $\mathbf{47}$                         & $188$     & $9.375\%$&$128$                &$\mathbf{6}$                               &$768$      &   $37.5\%$  &$0.189$&         $6.06$ \\\hline
    GTX 1080TI~\cite{gtx1080,turing,Techpower}                  &2017   &6.10           &$28$   & -&128    & 64&$4$      &   $\mathbf{47}$                         &  $188$    & $9.375\%$&$128$                &$\mathbf{6}$                               &$768$      &   $37.5\%$  &$0.354$&         $11.3$\\\hline
    RTX 2080TI~\cite{turing,Techpower}                          &2018   &7.50           &$68$   & -&64     & 32&$2$      &   $\mathbf{47}$                         &  $94$     &$12.5\%$ &$64 $        &$\mathbf{4}$                               &$256$      &   $25\%$  &$0.420$&         $14.2$ \\\hline
    GTX 3090 ~\cite{a102,Techpower}                             &2020   &8.60           &$82$   & - &128   &48 &$2$      &   $\mathbf{47}$                         &  $94$     &$8.33\%$ &$128$        &$\mathbf{4}$                               &$512$      &   $33.33\%$  &$0.556$&         $35.6$   \\\hline
    \end{tabular}
    \
    \begin{tabular}{|l|ccccc|cccc|ccccc|}\hline
    &\multicolumn{5}{c|}{{Shared Memory/SMX}}&\multicolumn{4}{c|}{L2 Cache}&\multicolumn{5}{c|}{{Global Memory}}\\
    GPU model               &(max)Size   &Bandwidth\cite{nvidia2019programming}      &Latency~\cite{wong2010demystifying}    &C & Min Occupancy   & Size  &Bandwidth      &Latency  &C/SMX    & Size       &Bandwidth      &Latency~\cite{zhang2022persistent}    &C/SMX & Min Occupancy    \\
                                &(KB)           &(B/clk)                                    &(cycle)    &       (B)         & (8B per access) & (MB)&   (GB/s) &(ns) &(B)& (GB)       &(GB/s)         &      (ns)   &        (B) &  (8B per access)  \\\hline
    \multicolumn{15}{|c|}{{Tesla/ Data Center GPUs}}   \\\hline            

    Nvidia Tesla K20~\cite{kepler}                              &$48$                 &       $256$ &       $\mathbf{47}$                   &$12032$&$73.44\%$  & $1.5$   &$\mathbf{287.69}$              &  $\mathbf{314.23}$  & $\mathbf{6026.72191}$  &$5$          &$208$            &     $\mathbf{480.80}$      &      6667 &    $42.19\%$    \\\hline
    Nvidia Tesla P100-PCIE~\cite{nvidia2017v100,amperewhite}    &$64$                 &       $128$ &       $24$~\cite{jia2018dissecting}   &$3072$ & $18.75\%$ & $4$ &$\mathbf{1540.09}$             &  $\mathbf{197.37}$ ($234$ cycle~\cite{jia2018dissecting})   &  $\mathbf{5459.71}$  &$12$         &$720$            & 4943         &        $\mathbf{384.49}$      &$31.25\%$   \\\hline
    Nvidia Tesla V100-SMX~\cite{nvidia2017v100,amperewhite}     &$96$                 &       $128$ &       $19$~\cite{jia2018dissecting}   &$2432$ &$15.63\%$  & $6$ &$\mathbf{2231.78}$ ($2048$bytes/clk)       &   $\mathbf{144.79}$ ($192$ cycle~\cite{jia2018dissecting})  &$\mathbf{4039.24}$&$16$         &$900$            &     $\mathbf{288.12}$      &     3241         &$20.31\%$ \\\hline
    Nvidia A100-PCIE~\cite{amperewhite}                         &$164$                &       $128$ &       $23/19$~\tnote{b}~\cite{abdelkhalik2022demystifying}       &   $2944/2432$~\tnote{b}         &$15.63\%/18.75\%$~\tnote{b}   & $40$    &$\mathbf{2543.62}$ ($5120$bytes/clk)           &  $\mathbf{144.88/314.26}$~\tnote{c} ($\mathbf{218/384}$ cycle) &$10335/18204$&$40$         &$1555$           &       $\mathbf{407.97}$    &       5874   &  $35.93\%$    \\\hline
    Nvidia H100-PCIE~\cite{nvidiah100}                          &$228$                &       $128$ &       -       &       - &-      & $50$        &-          &-    & - &$80$         &$2000$           &   -       &        - &-     \\\hline
    Nvidia H100-SMX~\cite{nvidiah100}                           &$228$                &       $128$ &       -       &       - &-      & $50$        &-          &-&-&$80$         &$3000$           &      -    &        -     &-\\\hline
    \multicolumn{15}{|c|}{{Workstation/ Consumer GPUs}}   \\\hline  
    GTX 980TI~\cite{gtx980,Techpower}                           &  $96$               &       $128$ &       $\mathbf{35}$      &       $4480$    &  $28.13\%$  & $3$        &     $\mathbf{748.15}$       &   $\mathbf{174.04}$      &   $\mathbf{5918.54}$    &$6$          &$336.6$   &  $\mathbf{299.20}$           &4578&$28.125\%$ \\\hline
    GTX 1080TI~\cite{gtx1080,turing,Techpower}                  &  $96$               &       $128$ &       $\mathbf{35}$      &       $4480$     & $28.13\%$   & $2.75$    &    $\mathbf{1204.59}$        &   $\mathbf{130.15}$     &    $\mathbf{5599.19}$   &$11$         &$484$   &    $\mathbf{235.38}$           &4068&$25\%$ \\\hline
    RTX 2080TI~\cite{turing,Techpower}                          &  $64$               &       $128$ &       $\mathbf{29}$      &       $3712$    &  $46.88\%$   & $5.5$     &   $\mathbf{1876.69}$         &    $\mathbf{111.80}$    &     $\mathbf{3085.50}$  &$11$         &$616$        &   $\mathbf{239.82}$       &2172&$28.125\%$ \\\hline
    GTX 3090~\cite{a102,Techpower}                              &  $96$               &       $128$ &       $\mathbf{29}$      &       $3712$    &  $31.25\%$   & $6$       &   $\mathbf{2041.82}$         &    $\mathbf{129.50}$   &     $\mathbf{3224.58}$  &$24$         &$936$        &   $\mathbf{267.45}$       &3052&$25\%$ \\\hline
    \end{tabular}
    \
    \begin{tabular}{|l|cc|cc|ccc|}\hline
    &\multicolumn{2}{c|}{{Shuffle}}&\multicolumn{2}{c|}{syncthreads}&\multicolumn{3}{c|}{{Latency of grid sync~\cite{zhang2020study}}}\\
    GPU model   &Throughput~\cite{nvidia2019programming}    & Latency~\cite{wong2010demystifying,zhang2020study}    &Throughput~\cite{nvidia2019programming}    & Latency~\cite{wong2010demystifying,zhang2020study}  &   &  &(max)    \\
    Block/SMX     &-    & -  &-& -    & $1$~\tnote{d}  & $\leq2$~\tnote{e}  &$32$    \\
    Thread/Block  &-    & -  &-& -   & $256$&  $\forall$ &  $64$)    \\
                &(op/clk)           &(clk)                               &(op/clk)           &(clk)                      & us & us                  & us     \\\hline
    \multicolumn{8}{|c|}{{Tesla/ Data Center GPUs}}   \\\hline            

    (kiev2 GPU0)Nvidia Tesla K20~\cite{kepler}                              &$32$ &$\mathbf{9}$                             &$128$  &$\mathbf{80}$                  &-&- &-              \\\hline
    (kiev6)Nvidia Tesla P100-PCIE~\cite{nvidia2017v100,amperewhite}         &$32$ &$31$~\cite{zhang2020study}   &$32$   & $\mathbf{138}$                &$1.83$~\cite{zhang2020study}& $1.77\sim3.52$~\cite{zhang2020study}&$28.42$~\cite{zhang2020study}   \\\hline
    (rwbc)Nvidia Tesla V100-SMX~\cite{nvidia2017v100,amperewhite}           &$32$ &$22$~\cite{zhang2020study}   &$16$   &$22$~\cite{zhang2020study}     &$1.50$~\cite{zhang2020study}&$1.43\sim3.49$~\cite{zhang2020study}&$24.51$~\cite{zhang2020study}       \\\hline
    (kiev0)Nvidia A100-PCIE~\cite{amperewhite}                              &$32$ &$\mathbf{26}$                &$16$   &$\mathbf{23}$                  &$\mathbf{1.21}$&$\mathbf{1.20\sim1.28}$& $\mathbf{18.02}$            \\\hline
    Nvidia H100-PCIE~\cite{nvidiah100}                                      &$32$ &-                            &-      &-                              &- &-&-       \\\hline
    Nvidia H100-SMX~\cite{nvidiah100}                                       &$32$ &-                            &-      &-                              &- &-&-     \\\hline
    \multicolumn{8}{|c|}{{Workstation/ Consumer GPUs}}   \\\hline  
    (kiev5)GTX 980TI~\cite{gtx980,Techpower}                                &$32$ &  $\mathbf{6}$                           &$64$   &$\mathbf{134}$&-&-&-  \\\hline
    (kiev1)GTX 1080TI~\cite{gtx1080,turing,Techpower}                       &$32$ &  $\mathbf{6}$                           &$64$   &$\mathbf{138}$&$\mathbf{1.06}$&$\mathbf{1.05\sim1.35}$&  $\mathbf{12.27}$ \\\hline
    (kiev2 GPU1)RTX 2080TI~\cite{turing,Techpower}                          &$16$ &  $\mathbf{4}$                           &$16$   &$\mathbf{22} $&$\mathbf{0.91}$&$\mathbf{0.86\sim1.57}$&  $\mathbf{5.07}$ (blk/SMX=16) \\\hline
    (roma7 GPU2)GTX 3090~\cite{a102,Techpower}                              &$32$ & $\mathbf{4}$                          &$16$   &$\mathbf{22} $&$\mathbf{0.63}$&$\mathbf{0.62\sim0.65}$&  $\mathbf{4.32}$ (blk/SMX=16) \\\hline
    \end{tabular}
    \begin{tablenotes}
    \item[a] Min occupancy is calculated by counting necessary warps to full fill concurrency (assuming thread level parallelism is the only means providing concurrency), divide it by the maximal active warps per stream multiprocessor. 
    \item[b] Load 23 cycle; Store 19 cycle.
    \item[c] We observed a clear near difference in latency between close hit and far hit. We are not sure how to use the full bandwidth of both slice of L2 cache.
    \item[d] The following research use this parameter setting. This research assume that it is possible to saturate the device with 256 threads per stream multi-processor.
    \item[e] The setting recommended by Zhang et al.~\cite{zhang2020study}.
    \end{tablenotes}
    \end{threeparttable}
    }
    \label{tab:stencil_speedups}
    % ~\tablefootnote{load 23 cycle; store 19 cycle}
\end{table*}


==> TABLE/gpuspecsofinterest.tex <==
\begin{table}[t]
    \centering
    \caption{GPU specs of interest in A100 for this paper. Details can refer to Nvidia documents~\cite{guide2022cuda,nvidiaa100}}
    % \resizebox{\columnwidth}{!}
    {%
    \footnotesize
    \begin{tabular}{|l|c|c|c|c|}\hline
    &$\mathbb{B}_{gm}$ &$\mathbb{B}_{sm}$&$\mathbb{THR}_{cmp}$\\  \hline 
    \textbf{Specs} &$1.555$ TB/s    &    $19.49$ TB/s &  $9.7$ TFLOPS/s      \\\hline
    \end{tabular}
    }
    \label{tab:specsintr}
\end{table}

==> ___GridTile.tex <==
% \section{Grid Level Tiling}
\section{One Tile at a Time}
\label{sec:gtile}
% As a practice of kicking Massive Execution away,
% \input{TABLE/KernelOverhead}
%However, grid level synchronization can have a high overhead. 
\subsection{Synchronization}
The introduction of grid level synchronization provides new opportunities for writing efficient GPU kernels. To quantify the overhead, we followed the research of Zhang et al.~\cite{zhang2020study} to test the overheads.
% Table~\ref{tab:overhead}. Kernel launch is usually considered an alternative to grid level synchronization~\cite{zhang2020study,Meng:2009:PMA:1542275.1542313}. As Table~\ref{tab:overhead} shows, 
Grid-level synchronization ($1.2$ us) has a lower overhead that that of a kernel launch ($2.2$ us) on the A100 GPU. 
% Using kernel launch for synchronization will wipe out all on-chip resources. Take 17.3MB of shared memory in A100 as an example. With $1555$ GB/s global memory bandwidth, we need about $12$ us to fill the whole shared memory. If we repeatedly load this amount of data onto the chip, without keeping the reusable data, we pay the cost of $12$ us for each load. 
\subsection{Tiling}
The introduction of grid level synchronization provides a new way to tile the domain: we tile the domain such that a single tile can scale up to use the entire shared memory capacity of the GPU. Next, we let the tile reside in shared memory while updating the cells for long enough time steps to amortize the overheads of initial loading and final storing. The final result for the tile is then stored on the device, and then we move to the next tile, i.e. the entire GPU is dedicated to computing only one single tile at any given time. Figure~\ref{Fig:gtb} shows how we do the overlapping tiling at the grid level.

One challenge of this method is to resolve the dependency between thread blocks in between time steps, since shared memory is only shared across threads belonging to the same thread block. Additionally, this method introduces of redundant computation at the grid level, as the light blue region in Figure~\ref{Fig:gtb} shows. That being said, as will be shown in the Evaluation section, the overheads of resolving the intra thread block dependencies and redundancy do not have significant effects on the performance gains. 

% Principle 2 is empirical, so the analysis of this section is empirical, using a 2D 5-point stencil implementation as an example. 

% A measurement is necessary to exchange the halo region. 
\subsection{Inter Thread Block Dependency}
Figure~\ref{fig:spblk}.c shows the dependency between thread blocks that we need to resolve. We use the bulk synchronous parallel (BSP) model to exchange the halo region and CUDA's grid-level barrier for synchronization. We transpose the halo region that originally did not coalesce to reduce the memory transactions.

\subsection{Overhead of the Temporal Halo Region}\label{sec:overheadgtile}
In order to resolve the dependency, we use overlapped tiling (readers can refer to Figure~\ref{fig:tblk}.a ). This introduces redundant computation. This topic is covered extensively in literature~\cite{Holewinski:2012:HCG:2304576.2304619,Meng:2009:PMA:1542275.1542313,10.1145/2830018.2830025}.

In fact, this overhead is not significant in our scheme of grid level tiling (where we use the entire GPU to process a single tile). As an example, at the grid level, our implementation of a 2D 5-point stencil we use a tile as large as $1152\times 1536$. We do very deep temporal blocking: we run $t=50$ time steps (which is over $5\times$ the highest number of time steps reported in the literature of temporal blocking on GPUs~\cite{DBLP:conf/cgo/MatsumuraZWEM20}). The valid region would shrink to $1052\times 1436$, which is $85.4\%$ of the loaded domain. Had we used thread block level overlapped tiling (as is typical in the literature of temporal blocking on GPUs), the shared memory of 164KB can hold at most $144^2$ of the 2D domain and running $t=50$ means only $44^2$ of the data is valid, which is only $9\%$ of the domain loaded. The pseudocode for the 2D 5-point Jacobian Stencil grid-level overlapped tiling is shown in Listing~\ref{listing:gtb}



\begin{figure}[t]
\centering
\includegraphics[width=0.9\linewidth]{FIG/GTB.pdf}
\caption{Overlapped titling at the CUDA grid level. $(gtile_x+HALO\times2)\times(gtile_y+HALO\times2)$ is the total size a device shared memory can hold. $(tile_x+halo\times2)\times(tile_y+halo\times2)$ is the total size a stream multiprocessor shared memory can hold. }
\label{Fig:gtb}
\end{figure}

\input{LISTING/grid_level_temporal_blocking}


==> ___Proposal1.tex <==
% \section{Cache hungry temporal blocking algorithm}
% \section{12.5\% is the occupancy we need}
% \section{Target plat}


% \subsection{Wrap up for stencil}


==> ___ResearceStarving.tex <==

\begin{figure*}[t]
\centering
\includegraphics[width=\linewidth]{FIG/StreamingDiff.pdf}
\caption{Different Streaming Schemes for 1 D 3-point Jacobi computation for temporally blocking. $ILP$: Instruction Level Parallelism.}
\label{Fig:streaming}
\end{figure*}
% \begin{figure}[t]
% \centering
% \includegraphics[width=\linewidth]{FIG/MemArrangement.pdf}
% \caption{On-chip memory (registers and shared memory) arrangement from the thread perspective, with t=2, ILP=2. (Lazy Streaming, Redundant Streaming, and Circular Schema are also enabled.)
% % \wahib{@Lingqi: "Before Execute" should be "Before Execution"; "After Execute" should be "After Execution"; "If suffer from register pressure" should "In case of regsiter pressure"}
% }
% \label{Fig:smarrange}
% \end{figure}


% \todo{revise this figure, hard to read hard to understand}

% \section{Resource-Scalable Optimizations}\label{sec:starving}
\section{Resource-Scalable Streaming}\label{sec:starving}

In this section, we propose several optimizations for Streaming that can scale with the increase in resources, i.e., cache and registers.

\subsection{Prefetching}\label{sec:prefetch}% With Asynchronous Shared Memory Copy}
Prefetching is a well-documented optimization. The readers can refer to~\cite{rawat2019optimizing} for hints. We use the new asynchronous shared memory copy API to conduct prefetching. These APIs require additional shared memory space for buffering. By default, we use this optimization. 

\subsection{Lazy Streaming}\label{sec:lazystreaming}
Figure~\ref{Fig:streaming}.a shows serial streaming in 1D 3-point Jacobi calculation. Some of the data are cached in on-chip memory. We then load one data point $ld1$ and use it to compute the three steps we temporally block, then finally store the result $st1$ on the device memory. Meanwhile, the intermediate result would be cached for computation of $ld2$. The problem of serial streaming is its long chain of dependencies in operations. This long chin of dependencies would gradually convert the stencil computation from being throughput bound to become latency bound problem.%, even though the dependency only existed in on-chip resources. 

%So, the update of a point is postponed. 
We propose \emph{lazy streaming}. The basic idea is that we delay the processing of a domain cell until all domain cells required to update the current cell are already updated. Otherwise, we would pack the planes that include the current domain cell and cache it in on-chip memory. As Figure~\ref{Fig:streaming}.b shows, the computation of \textit{st1} is postponed until the three points of the previous time steps are updated. 
 
The benefit of using Lazy Streaming is not significant in 1D stencils. In 2D or 3D stencils, we replace the points in Figure~\ref{Fig:streaming} with 1D or 2D planes for 2D or 3D stencils. The planes usually involve inter-thread dependency, which makes synchronizations unavoidable (warp shuffle when using registers for locality~\cite{chen2019versatile, sat} or thread block synchronization when using shared memory for locality~\cite{maruyama2014optimizing}). However, synchronizations have overhead~\cite{zhang2020study}. Lazy streaming can ideally reduce the synchronization to one synchronization per blocked plane. 

%just like procrastination pile-up works
The trade-off of using Lazy Streaming is that it needs more space to cache the intermediate data. We further discuss resource consumption when composing lazy streaming in N.5D tiling in Section~\ref{sec:smusageana}.

\subsubsection{Increasing Instruction Level Parallelism}
Lazy Streaming can sustain high $ILP$ since it reduces the dependencies to the minimum possible. There could be cases when additional $ILP$ is necessary, that is, more data load instructions are needed to provide enough concurrency for saturating the global memory bus. One option is to update more domain cells per thread (Items Per Thread, $IPT$) in the streaming direction. Figure~\ref{Fig:streaming}.c shows an example of doubling the ILP in lazy streaming.%$ The total memory consumption including IPT is: $(IPT+2\times rad)\times t$.

% \subsection{Redundant Streaming with Registers}
\revision{\subsection{Register Streaming}\label{sec:redundant}}

At low occupancy, we obtain a large number of registers and shared memory per thread. Therefore, by reducing the occupancy we can afford to redundantly store intermediate data in both the registers and the shared memory. Streaming w/ caching in shared memory is discussed in STENCILGEN~\cite{rawat2018domain}. Streaming w/ caching in the registers is discussed in AN5D~\cite{DBLP:conf/cgo/MatsumuraZWEM20}. By caching in both shared memory and registers, we get benefits from both components. We can reduce shared memory access times to minimum by using registers first (in comparison to AN5D) while also reducing the necessary synchronizations when using only shared memory (in comparison to STENCILGEN). 


\subsection{Caching Space Reuse}
Finally, we propose a simple optimization that slightly reduces the caching space requirements. As Figure~\ref{Fig:smarrange} shows, in streaming, some data would expire. In a single computation of the data in $reg_0$, $reg_1$, $reg_2$, the data in $reg_0$ expires after the cell update has been concluded. We use this location to hold the result as: $reg_0=COMPUTE(reg_0,reg_1,reg_2)$. We do the same optimization also for data held in shared memory. In Listing~\ref{Fig:streamingreuseschema}, line 14 reuses the same input location in line 15 as an output destination. We use this optimization by default in EBISU.




==> ___WrapperUp.tex <==
% \section{EBISU: Epoch (temporal) Blocking for Iterative Stencils, with Ultracompact parallelism}\label{sec:cosfmodel}
\section{EBISU: Analysis of Design Choices}
%\label{sec:designchoice}
% \input{TABLE/ParamaterUsed}
% \input{TABLE/gpuspecsofinterest}

% We wrap up the optimizations and propose a novel temporal blocking approach, EBISU (/e bi: s/).%: tEmporal Blocking with mInimal neceSsary parallel execUtion.

% EBISU is essentially an extension of N.5D temporal blocking. We spatially block in one dimension (or two dimensions in 3d stencils) and streaming in the remaining dimension. For the spatial tiling part, we implemented two variants: overlapped tiling and grid-level tiling. 

% Note that EBISU consists of purely assembling the optimizations we proposed in Section~\ref{sec:starving} and Section~\ref{sec:gtile}. So, in this section, we only briefly discuss the optimization used and do not elaborate implementation details, i.e. how we assemble the existing optimizations. The design decision is summarized at Table~\ref{tab:designDecision}. 

In this section, we focus mainly on using an analytical model to support our design decisions. We use the giga-cells updated per second (GCells/s) as the metric for stencil performance~\cite{DBLP:conf/cgo/MatsumuraZWEM20,chen2019versatile}. The analysis is targeted at the A100 GPU, while it can be generalized to any GPU platform by adjusting the model parameters (Table~\ref{tab:designDecision} summarizes our findings on design choices). 

\todo{The parametric study is important since the analytical model does not derive the best configuration of EBISU, especially for the temporal blocking depth.}

\subsection{Parameterizing for Size of Spatial Tiles and Depth of Temporal Blocking}
In this paper, we are less concerned with whether the bottleneck is shifted to computation or to the cache bandwidth. To simplify the discussion, in this section, we assume that the optimization goal is to shift the bottleneck of the stencil from global memory to shared memory. This assumption is true for most of the star-shaped stencils~\cite{DBLP:conf/cgo/MatsumuraZWEM20}. Accordingly, we have: 
\begin{equation}\footnotesize
    \frac{{a}_{sm}\times t}{\mathbb{B}_{sm}}\times{\mathbb{D}_{sm}} \geq \frac{{a}_{gm}}{\mathbb{B}_{gm}}\times\mathbb{D}_{gm}
    \label{eqt:basidassume}
\end{equation}

\subsubsection{Thread Block 2.5D Temporal Blocking}\label{sec:smusageana}
% Overlapped N.5D tiling is widely discussed in existing literature~\cite{DBLP:conf/cgo/MatsumuraZWEM20,rawat2018domain,nguyen20103}. We do not modify the implementation principles. We only use the Lazy Streaming and Redundant Streaming to replace the Streaming implementations, and use Cycle Schema (compute address) to arrange shared memory address.

As Section~\ref{sec:cost2d5pt} showed, the overlapped 2.5D temporal blocking has a lower overhead. We optimize only for a sufficiently large temporal blocking size to shift the bottleneck. 

% This section, we, under the back ground of N.5D temporal blocking, analyze the resources consumption when composing our resource starving optimizations with overlapped tiling.

% We use 2D 5-point Jacobian Stencil as an example. 
% 
% \subsection{Resources usage analysis: 2D stencils}\label{sec:resourcesls}
\noindent\textbf{What Depth of Temporal Blocking Do We Need?}
To simplify the discussion, we dismiss the effect of the halo region. Ideally, we have $\mathbb{D}_{sm}=\mathbb{D}_{gm}$. In A100, $\mathbb{B}_{gm}=1555$ GB/s, $\mathbb{B}_{sm}=19.49$ TB/s. In our 2D 5-point implementation, $\mathbf{a}_{gm}=2$ (assuming perfect caching), $\mathbf{a}_{sm}=3$. According to Equation~\ref{eqt:basidassume}, we have $t\geq8.4$. In $t=9$, we observe the performance $\mathbb{P}_{tbtile}{(t=9)}=455$ GCells/s. We can achieve slightly better performance at $t=12$, where $\mathbb{P}_{tbtile}{(t=12)}=482$ GCells/s. There is only $6\%$ difference in performance. The slight inaccuracy might come from the fact that, on average, the global memory accesses per data point is not perfectly cached. 

Nevertheless, in overlapped tiling, we only need temporal blocking to be deep enough to shift the bottleneck. 


\noindent\textbf{Shared Memory: How Much Capacity Do We Need?}
% 
% We base our analysis on 2D 5-point Jacobian stencil. However, it can be generalized to other stencils. 

% Assume that we temporal blocking of $t$, and spacial blocking of $T$. Spacial blocking depends on the size of the building block, i.e. $bdim$, $ILP$, and the order of the stencil $rad$. 

As Figure~\ref{Fig:smarrange} shows, the total shared memory consumption $SM_{size}$ is:
% \todo{How to express tiling in streaming direction}
\begin{equation}\footnotesize
    \mathbb{S}_{SM}=(t\times(rad+IPT)+IPT)\times PLANE\times \mathbb{S}_{Cell}
    \label{eqt:smsize}
\end{equation}
% Accordingly, we have:
% \begin{equation}\footnotesize
    % t = \tfrac{SM_{size} - ILP\times bdim \times sizeof(Data)}{(rad\times2+ILP)\times bdim\times sizeof(Data)}
% \end{equation}
% In A100, $SM_{size}=164$KB.

% \noindent\textbf{2D 5-point Jacobian} 
In our 2D 5-point Jacobian implementation, $PLANE=tile_x=258$, $IPT=4$, $rad=1$. From the previous section, our aim is to achieve $t>=9$ or $t=12$. We have: $ \mathbb{S}_{SM}(t=9)=98$ KB and $ \mathbb{S}_{SM}(t=12)=128$ KB. 

To also consider the overhead of using the circular schema, the range of the address space is $range\_basic=t\times(rad+IPT)+IPT$. In $t=9$ or $t=12$, we need $range=64$ to implement the circular structure. In this situation, $ \mathbb{S}_{SM}(t=12|circular\ schema)=128$ KB.

\subsubsection{Grid 3.5D Temporal Blocking}\label{sec:gtbdpt}
Unlike overlapped temporal blocking, the main overhead of grid level tiling is grid level synchronization. So naturally, we run the tiling as large as possible to amortize the overhead of synchronization. 

\noindent\textbf{An Empirical Analysis: How Deep Do We Go?}
The search space for grid 3.5D temporal blocking is large. Both the choice of partial tiling and the depth of temporal blocking influence performance. For simplicity, in this research, we first choose a spatial blocking size that is large enough while easy to program, then run the temporal blocking as deep as possible, to amortize the overhead of using grid level synchronization. 

\noindent\textbf{Thread Block Level Spatial Blocking: How Large Do We Go?}
For simplicity, we assume that the very first plane loaded and the last plane stored have already been amortized. Then, for global memory access, we only focus on the halo region. According to Equation~\ref{eqt:basidassume}, we have:
\begin{equation}\footnotesize
    \frac{tile_x\times tile_y \times{a}_{sm}}{\mathbb{B}_{sm}} > \frac{(tile_x+tile_y)\times2\times{a}_{gm}\times rad}{\mathbb{B}_{gm}}
\end{equation}

We assume that $tile_y=tile_x$. So, we can get: 
\begin{equation}\footnotesize
    tile_y=tile_x >{\frac{4\times {a}_{gm}\times \mathbb{B}_{sm}}{{a}_{sm}\times\mathbb{B}_{gm}}}\times rad
\end{equation}

In our 3d7pt implementation, ${a}_{gm}=2$, ${a}_{sm}=4.5$. We have $tile_y=tile_x\geq 22.3$. For convenience, we use $32\times32$ (also fitted to the Minimal Necessary Parallelism that saturates the device as Section~\ref{sec:parallelismneed} discussed). 

Most of the 3D stencils we studied only need thread block tiling of $32\times32$ to hide the latency of the access halo region, except 3d13pt. We still use $32\times32$ for simplicity. %because, in our experiment, double the spatial tiling reduces the temporal blocking size so much that it has a lower performance compared to using $32\times32$. 


% \subsection{Design Choice for EBISU}
% With a systematic analysis of different types of stencil in A100, we summarize the design decision for EBISU in Table~\ref{tab:designDecision}.% We used prefetching and data reused by default, but we didn't include them in the Table.

% \input{TABLE/designDecision}
% After a systematic analysis on different types of stencils in A100, we use overlapped 2.5D stencils in 2D stencils and grid level 3.5D tiling in 3D stencils for EBISU. Note that similar analysis should be conducted for different stencils in different hardware platforms. 

% \footnote{A building block in this paper is a minimal combination of threads and instruction level parallel that has enough work to saturate the device} 

==> ____Proposal2.tex <==

% Traditionally, GPU programming only consider the workload in a thread block level. In grid level, or kernel level, researchers just greedily chasing massively available workloads. In order that this layer of tiling benefit performance, we propose that the size of the tiling is large enough to use the on-chip resources and small enough such that the memory accesses to global memory are highly possible fitted to L2 cache. The grid level synchronization also provide additional flexibility in programming for grid level tiling. 

% Additionally, the grid level synchronization make
% \subsection{Grid level synchronization}

==> ____RelatedWorks.tex <==
\section{Related works}
% In this section we firstly introduce the background of stencil computation and temporal blocking. Then we discuss the limitation in current the state of the art temporal blocking implementation in GPU. 

% \subsection{Spatial Blocking Stencil~\cite{irigoin1988supernode,Wolfe:1989:MIS:76263.76337}}
% In spatial blocking on GPUs, we split the domain into sub-domains, where each thread block can load its sub-domain to the shared memory to improve the data reuse. In the meantime, we require redundant data accesses at the boundary of the thread block to data designated for adjacent thread blocks. 

% \subsection{Temporal Blocking Stencil~\cite{DBLP:conf/cgo/MatsumuraZWEM20,rawat2016effective}}
% In iterative stencils, each time step depends on the result of the previous time step. One could advance the solution by combining several time steps. The temporal dependency, in this case, is resolved by using a number of halo layers that match the number of combined steps. The amount of data that can be computed depends on the stencil radius ($rad$) and the number of time steps that are combined ($b_t$). In overlapped temporal tiling~\cite{Holewinski:2012:HCG:2304576.2304619,Krishnamoorthy:2007:EAP:1250734.1250761,Meng:2009:PMA:1542275.1542313}, this region can be represented as {$2 \times b_t\times rad$} ($halo$ region). Methods based on this kind of blocking are called \textit{overlapped temporal blocking} schemes. 

% StencilGen~\cite{rawat2018domain} and AN5D~\cite{DBLP:conf/cgo/MatsumuraZWEM20} are two state of the art temporal blocking implementation in GPU. StencilGen only implemented shallower temporal blocking (2-4 time steps). AN5D implemented deeper temporal blocking number, but it suffer from register pressure in double precision and in high order stencil.



% \subsection{Limitation of state of the arts}
% \subsubsection{Register pressure}
% Register pressure commonly occur in temporal blocking~\cite{DBLP:conf/cgo/MatsumuraZWEM20} and high order stencil~\cite{stock2014framework}. Many researchers~\cite{rawat2018associative,Rawat:2018:ROS:3200691.3178500} efforts in resolve issues in high order stencils. However, the register pressure in temporal blocking is hard to resolve with existing methods\todo{add cite and check}. GPU temporal blocking usually require a deep time steps such that the method can effectively move the bottleneck from global memory to cache. However, in temporal blocking, the dependency between register increase as blocked time steps increase. So in deep temporal blocking situation, usually before the register spill, registers are not enough to support parallelism such that the program need to wait the register become available to further issue instructions. We consider this as \textbf{register bound} because the performance could automatically increase if the amount of registers increase. 

% %Some efforts related to register allocation, others integrate integrate register allocation and instruction scheduling. Also some researches explicitly optimize register usage in high order stencils. 


% %  So we believe register pressure is one of the barrier that stop GPU temporal blocking methods to go deeper temporal blocking. Register pressure also exists in high order stencils, many researches working on reducing register usage to increase performance. 

% % However, with the knowledge that GPU and endure even lower occupancy to saturate the device, and lower occupancy provide more register per thread. \textbf{Proposal:} we propose to optimize stencil for lower occupancy to release the register pressure. 

% \subsubsection{Increasing halo to resolve dependency}
% Overlapped tiling is widely used in temporal blocking~\cite{rawat2018domain,DBLP:conf/cgo/MatsumuraZWEM20}. However it has high overhead as the temporal time step increased. N.5D tiling~\cite{rawat2018domain,DBLP:conf/cgo/MatsumuraZWEM20} is applied to alleviate such overhead. Yet its overhead is still significant as we analyze in the Performance Analysis section. Considering a 32x32xN tiling for 3d7pt stencil, after 4 time steps the redundant computation is about 43.75\%. One alternative is to use complex shape tiling, i.e. diamond blocking~\cite{bondhugula2016diamond} or hexagonal tiling~\cite{grosser2014hybrid}. Mapping this shape to hardware while ensuring concurrency is not a trivial job. For example, consider a 2d5pt stencil with diamond tiling. In each blocked time step it need to load or store 2 data, which is not enough to provide enough concurrency to saturate the device. Malas et. al.~\cite{malas2015multicore} provided a good hint, to only use diamond tiling in one dimension, while use another dimension to provide concurrency. It shows very promising performance in CPU. But this method consume too much cache so that not yet applicable in current GPU. (Ref to performance analysis). 
% ---



==> ___architecgtureinsight.tex <==
\section{GPU evolution high lights that motivate this research}

In this section, we firstly introduce the background of the CUDA programming model and Nvidia GPU architecture, and we introduce the new feature highlights. We show the trends in GPU architectures by statistical data as well as microbenchmarks. Finally, we summarize the highlights that inspire this research.
% % Then we highlight the trends in GPU architectures, that we believe would benefit general GPU programming and especially could benefit stencil.
% \subsection{CUDA programming model and Nvidia GPU architecture}
% % \todo{rephrazing}
% The CUDA programming model includes: the base execution unit, thread; 32 threads grouped into a block of schedule units, warps; Several warps grouped together into a thread block unit; and thread block unit further unit up to be a grid. 

% When mapping the programming model to the GPU architecture, the CUDA driver maps the thread block to a stream multiprocessor (SM). The mapping abides by the rules of the limitation of resources. For example, at most 8 thread blocks and at most 2048 threads can reside concurrently in a stream multiprocessor. Also, there is a limitation in the total amount of registers and shared memory in a stream multiprocessor. The more these resources required by a thread, or a thread block, the fewer concurrently running threads or thread blocks are allowed. 


% % \input{TABLE/gpu_specs}
% % When the hardware can not provide additional resources, additional parallelism from software, i.e. more thread blocks or more kernels, can only run serially. We consider this scenario as \textbf{device saturated}. 

% \subsubsection{Explicit synchronization primers.}
% From P100~\cite{nvidia2019programming}, Nvidia introduced cooperative group APIs to provide a hierarchical of synchronizations in addition to thread block synchronization. The new grid level synchronization provide additional choice for program. Zhang et. al.~\cite{zhang2020study} shows that these APIs are mature enough for productive usage.

% \subsubsection{Asynchronous shared memory copy.}
% A100 (2020) further introduced APIs to copy data from global memory to shared memory, without blocking. Martin et. al.~\cite{svedin2021benchmarking} used this API and showed that this API mainly benefits low-arithmetic intensity kernels. 


\subsection{Scratchpad memory capacity}
\begin{figure}[t]
\centering
 \includegraphics[width=0.48\textwidth]{FIG/SharedMemSize.pdf}
 \caption{Trends of shared memory capacity}
 \label{fig:sm}
\end{figure}
We plot the total volume of scratchpad memory in latest GPU in Figure~\ref{fig:sm}. The total volume of scratchpad memory amount is over $24.7$x larger in last decades. Even in single stream multi-processor, the capacity of scratchpad memory in A100 is about $3.4$x larger compared with K20 released about a decades before. Worth mentioning that in H100~\cite{nvidiah100}, per stream multiprocessor shared memory capacity would be $228$ KB, which makes the total shared memory capacity be $42.0$x larger than the capacity of K20. 


\begin{figure}[t]
\centering
 \includegraphics[width=0.48\textwidth]{FIG/OccupancyTrends.pdf}
 \caption{Minimal occupancy to achieve peak performance}
 \label{fig:occupancy}
\end{figure}

% \begin{figure}[t]
% \centering
%  \subfloat[FFMA and DFMA] {
%  \includegraphics[width=0.24\textwidth]{FIG/PerformancePerOccupancy.pdf}
%  \label{fig:occcmp}
%  }
%  \subfloat[Bandwidth of shared memory (left axle) and global memory (right axle)] {
%  \includegraphics[width=0.24\textwidth]{FIG/BandwidthPerOccupancy.pdf}
%  \label{fig:occbwd}
%  }
%  \caption{Achievable performance with 1 warp per stream multiprocessor }
%  \label{fig:occupancyachievable}
% \end{figure}



\subsection{Lower occupancy required to saturate the device}
Volkov was the first to investigate the parallelism that influences performance~\cite{volkov2010better}. They first find the minimal parallelism that can saturate the device. He points out that instruction level parallelism (ILP) is an alternative method for providing parallelism, beside thread level parallelism (TLP). Then, he optimizes the kernel based on such value, which results in a lower occupancy while higher performance. %Though compiler usually supports automatic ILP, it is hard  
However, this research was conducted more than a decade ago. In this subsection we follow Volkov's research to microbenchmark the Data Center GPU in the last ten years to inspect the parallelism required to saturate the device. 

\subsubsection{ILP=1}
For simplicity, we first consider only TLP and directly port parallelism to the required occupancy. We inspect DFAM (double precision multiply and add operation) as an example of compute bound kernels. We inspect the shared memory and global memory as an example of memory-bound kernels. For memory related results, we assume $8$B per access requires. Figure~\ref{fig:occupancy} shows the result. We can observe clear trends in decreasing required minimal occupancy over years. $20.31\%$ in V100 and $36\%$ in A100 are necessary to saturate the device with all the components that we are interested in. However, in K100, the minimal occupancy was $73.4\%$. 

\subsubsection{ILP=4, Occupancy=12.5\%}
\begin{figure}[t]
\centering
 \includegraphics[width=0.48\textwidth]{FIG/AchievedBandwidth.pdf}
 \caption{The performance of oversubscription and 1/8 occupancy. In latest GPUs, it is easy to achieve 90\% of oversubscription performance with lower occupany}
 \label{fig:bandwidth}
\end{figure}
\begin{figure}[t]
\centering
 \includegraphics[width=0.48\textwidth]{FIG/RegisterConsumed.pdf}
 \caption{The register usage of oversubscription and 1/8 occupancy. Lower occupany with ILP consume less registers.}
 \label{fig:register}
\end{figure}
% \todo{Not yet conducted benchmark}
Many optimizations are based on ILP that can tolerate even lower occupancy~\cite{kronbichler2019multigrid,zachariadis2020accelerating,swirydowicz2019acceleration,merrill2016merge}. We run the STREAM test with ILP=4 and $occupancy=12.5\%$ in this subsection. The result is shown in Figure~\ref{fig:bandwidth}. The result shows that 12.5\% occupancy can achieve 90\% of performance compared to the oversubscription version in the latest GPUs. Figure~\ref{fig:register} shows that 12.5\% occupancy consumed far less reigsters compared with oversubscription. 
% We try to inspect how much performance we can achieve with $occupancy=12.5\%$ (or 256 threads per stream multiprocessor). We in this part use a simple STREAM kernel of $a=b*b$ to represent a memory-bound kernel. We increase the multiply $100$ times to represent compute-bound kernel.

\subsection{Device-wide synchronize}
Zhang et al.~\cite{zhang2020study} conducted a comprehensive study on different level of GPU synchronizations. Yet they didn't include A100 GPU. We adjust their benchmark codes and test the performance in A100 GPU. We are curious about how the performance of device-wide synchronization migrates, so we put the grid synchronization results and implicit barrier (kernel launch overhead as they suggested) in the same figure. We intent to use 12.5\% occupancy, so we do not report other parameter settings that might introduce contention and have high overheads. Figure~\ref{fig:syncoverhead} shows the results. The result shows that the latency of grid synchronization is decrease over time and in A100, its overhead is even smaller than the overhead of kernel launch. This means that using grid synchronization in A100 to replace kernel launch is more profitable.

\begin{figure}[t]
\centering
 \includegraphics[width=0.48\textwidth]{FIG/SyncOverhead.pdf}
 \caption{Minimal occupancy to achieve peak performance}
 \label{fig:syncoverhead}
\end{figure}


% Then we assume that only one warp per stream multiprocessor was launched to use the components of interest, we also plot its achievable performance over different platforms. We plot computation related data in Figure~\ref{fig:occcmp} and memory related in Figure~\ref{fig:occbwd}. We can see a clear trends that the power of warps is also increasing over years.% One exception is the global memory access in A100 seems stays the same level as V100.%, which won't influence the general trend. 

%We can see the power of warps is also increasing over years. On interesting finding is that warps in V100 seems be more efficient in global memory access. 
% Following Volkov's research, we microbenchmarks the Data Center GPU in last ten years to see if the devic
% understand the trends of minimal occupancy required to achieve peak performance. We inspect FFMA, DFAM as an example of compute bound kernels. We inspect the bandwidth of shared memory and global memory as an example of memory bound kernels. For bandwidth results, we assume $8$B per access requires. Figure~\ref{fig:occupancy} shows a clear drop in required occupancy in last 10 years. 

% We this knowledge, we anticipate that cache 


% \subsection{Discussion}

% \subsection{GPU new features}
% \subsubsection{Explicit synchronization primers.}
% From P100~\cite{nvidia2019programming}, Nvidia introduced cooperative group APIs to provide a hierarchical of synchronizations in addition to thread block synchronization. The new grid level synchronization provide additional choice for program. Zhang et. al.~\cite{zhang2020study} shows that these APIs are mature enough for productive usage.

% \subsubsection{Asynchronous shared memory copy.}
% A100 (2020) further introduced APIs to copy data from global memory to shared memory, without blocking. Martin et. al.~\cite{svedin2021benchmarking} used this API and showed that this API mainly benefits low-arithmetic intensity kernels. 

\subsection{Summary}




==> ___buildingblock.tex <==
% \section{Compact Occupancy for On-chip Resources}\label{sec:lowoccupancy}
\color{red}
\section{Temporal Blocking Constructed from Building Blocks with Compact Parallelism}\label{sec:lowoccupancy}

\subsection{Necessary Parallelism}
The analysis of this section is an extension of Volkov's research~\cite{volkov2010better}. We based our analysis on Little's law, too. Little's Law use Latency $\mathbb{L}$ and Throughput $\mathbb{THR}$ to infer the concurrency $\mathbb{C}$ of the given hardware:
\begin{equation}\footnotesize
     \mathbb{C}=\mathbb{L}\times\mathbb{THR}
\end{equation}

$\mathbb{L}$ of an instruction can be gathered by common microbenchmarks~\cite{wong2010demystifying,mei2016dissecting}. $\mathbb{THR}$ of an instruction can refer to nvidia documents~\cite{guide2022cuda,nvidiaa100}.

As long as the Parallelism $\mathbb{PAR}$ provided by the software is larger than the concurrency provided by the hardware, we consider that the software saturate the hardware:

\begin{equation}\footnotesize
     \mathbb{PAR}\ge\mathbb{C}
\end{equation}

There are two ways of providing parallelism: Thread Level Parallelism ($TLP$) and Instruction Level Parallelism ($ILP$), according to Volkov's research~\cite{volkov2010better}. Accordingly, we have:

\begin{equation}\footnotesize
     \mathbb{PAR}={TLP}\times{ILP}
\end{equation}

Note that we veered off Volkov's path from this place. Instead of maximize the parallelism with the combination of $ILP$ and $TLP$, we aim to find a minimal combination of $TLP$ and $ILP$ that saturates:

\begin{equation}\footnotesize
     {TLP}\times{ILP}=\mathbb{PAR}\ge\mathbb{C}=\mathbb{L}\times\mathbb{THR}
\end{equation}

% Occupancy is usually considered a representation of Parallelism. But it is only true when the program only rely on TLP for Parallelism. Basically, $Occupancy=12.5\%$ when $TLP=256$. In this case, if $ILP=1$, then $\mathbb{P}=256$.

To maintain a certain level of parallelism, we can reduce the occupancy ($TLP$) and increase $ILP$ at the same time. We reduce the occupancy to a point that it will not increase the resources per thread blocks. In current hardware (A100), further reduce occupancy to less than $12.5\%$ will not increase the available register per thread~\cite{guide2022cuda}. So, we set our aim at $Occupancy=12.5\%$ or $TLP=256$. %In this case, we need $ILP=4$.

% \subsubsection{Minimal Sufficient Parallelism: A Case Study On the STREAM Kernel}
% We consider a $a=b$ STREAM kernel~\cite{mccalpin1995stream} . This kernel is bound by the memory bandwidth. According to Little's Law, $35.93\%$ of occupancy is necessary with $ILP=1$. In $ILP=4$, we only need $10\%$ occupancy. %In this case, Section~\ref{sec:motiveOver} showed that in STREAM kernel, $Occupancy=12.5\%$ with $ILP=4$ can provide $91\%$ of the performance compared with maximal occupancy version (oversubscription) of the same implementation.

% We used 256 thread per thread blocks and ILP = 4 as building block to build STREAM Kernel. As a result, the performance of Oversubscription with such building block is $P_{Occupancy=100\%}=1291$ GB/s. On the other hand, if we reduce the occupancy to $1/8$, we get: $P_{Occupancy=12.5\%}=1172$ GB/s. The performance difference is small ($9\%$). 

% This case study reassure that Little's Law can help figuring out the setting for the choice of building block. This case study also bring up a question: is it worthwhile to use $7/8$ for improving $9\%$ of 
% In this simple way, we trade $9\%$ of performance for freeing $87.5\%$ of on-chip resources. 

\subsection{Extended Building Block}\label{sec:buildingblock}
% In the GPU, the warp is a schedule units. Program in GPU without the aware of warp might not get sufficient performance. Thus, by default, warp is a building block for GPU program. In this sense, we just extend the building block of GPU programming to a larger unit. %More specifically, we define a combination of thread-level parallel and instruction-level parallel as a programming unit, then we build implementation with this building block.

In this research, we focus on double precision global memory access, shared memory access, and DFMA, all of which are basic of stencil computation. based on Little's Law~\cite{volkov2010better}, $ILP=4$ and $Occupancy=12.5\%$ ($TLP=256$) provides enough parallelism for all three operations. We set this as a building block for our implementation. 

In the 2d stencil, we use ILP in the stream direction (Details refer to Section~\ref{sec:lazystreaming}).

In 3d stencils, we compose $256\times4$ to do spatial tiling as $32\times32$. 

% \section{Temporal Blocking Constructed from Building Blocks with Compact Parallelism}\label{sec:lowoccupancy}
% The state-of-the-art temporal blocking work by Matsumura et al.~\cite{DBLP:conf/cgo/MatsumuraZWEM20} (AN5D) reported that their deep temporal blocking with a dimension being streamed in registers would suffer from register pressure~\cite{DBLP:conf/cgo/MatsumuraZWEM20}. However, we found that their maximum register usage is 96 registers per thread, while the maximum number of registers available per thread is 256~\cite{guide2022cuda}. The number of registers per thread in AN5D is restricted in order to ensure high occupancy. That is since for AN5D the algorithm is first designed, then the occupancy (parallelism) is tuned for performance.

% In this paper, we use the opposite approach: we start with a building block set to the minimal number of threads and instruction level parallelism that would fully utilize the device. Next, we stay with such setting to design the whole temporal blocking algorithm. Because the building block itself has already saturated the device, we can assume that implementations built from the building block can provide enough parallelism to saturate the device. In this sense, we do not further optimize the algorithm to expose parallelism; instead, we optimize the algorithm for resources scalability. It is worth noting that this approach is inspired by the work of Volkov et al.~\cite{volkov2010better}. 


% % \subsection{Kick Oversubscription (Max Parallelism) away}\label{sec:motiveOver}
% % \subsubsection{Overview of Oversubscription}
% % Generally, oversubscription means that the execution of thread blocks larger than the hardware limit, then the dynamic scheduler is leveraged for workload assignment. This method automatically achieves the maximum occupancy that the device can support. So, this principle involves two assumptions: 1. dynamic scheduler always performs well; and 2. highest available occupancy always benefits performance. However, many by-passsing schedulers~\cite{aila2009understanding,chen2010dynamic,ma2020rammer} shows that dynamic scheduler not always outperform manual efforts. Furthermore, Volkov~\cite{volkov2010better} shows that low occupancy might outperform higher occupancy with the help of Instruction Level Parallelism (ILP). Additionally, ILP is now summarized as a principle in the CUDA programming guide~\cite{guide2022cuda} now. 

% % \textbf{However, existing researches, including Volkov's research~\cite{volkov2010better}, are still chasing the maximal available occupancy hardware can provide.} In this research, we extend the definition of Oversubscription as: \textbf{Oversubscription happended when launched thread blocks exceed the concurrency provided by the hardware.} Because the thread blocks launched, even thought concurrently reside in the hardware, might not use resources efficiently when Oversubscription happened.% and suffer from Diminishing Marginal Returns.

% \subsection{Necessary Parallelism}
% The analysis of this section is an extension of Volkov's research~\cite{volkov2010better}. We based our analysis on Little's law, too. Little's Law use Latency $\mathbb{L}$ and Throughput $\mathbb{THR}$ to infer the concurrency $\mathbb{C}$ of the given hardware:
% \begin{equation}\footnotesize
%      \mathbb{C}=\mathbb{L}\times\mathbb{THR}
% \end{equation}

% $\mathbb{L}$ of an instruction can be gathered by common microbenchmarks~\cite{wong2010demystifying,mei2016dissecting}. $\mathbb{THR}$ of an instruction can refer to nvidia documents~\cite{guide2022cuda,nvidiaa100}.

% As long as the Parallelism $\mathbb{PAR}$ provided by the software is larger than the concurrency provided by the hardware, we consider that the software saturate the hardware:

% \begin{equation}\footnotesize
%      \mathbb{PAR}\ge\mathbb{C}
% \end{equation}

% There are two ways of providing parallelism: Thread Level Parallelism ($TLP$) and Instruction Level Parallelism ($ILP$), according to Volkov's research~\cite{volkov2010better}. Accordingly, we have:

% \begin{equation}\footnotesize
%      \mathbb{PAR}={TLP}\times{ILP}
% \end{equation}

% Note that we veered off Volkov's path from this place. Instead of maximize the parallelism with the combination of $ILP$ and $TLP$, we aim to find a minimal combination of $TLP$ and $ILP$ that saturates:

% \begin{equation}\footnotesize
%      {TLP}\times{ILP}=\mathbb{PAR}\ge\mathbb{C}=\mathbb{L}\times\mathbb{THR}
% \end{equation}

% % Occupancy is usually considered a representation of Parallelism. But it is only true when the program only rely on TLP for Parallelism. Basically, $Occupancy=12.5\%$ when $TLP=256$. In this case, if $ILP=1$, then $\mathbb{P}=256$.

% To maintain a certain level of parallelism, we can reduce the occupancy ($TLP$) and increase $ILP$ at the same time. We reduce the occupancy to a point that it will not increase the resources per thread blocks. In current hardware (A100), further reduce occupancy to less than $12.5\%$ will not increase the available register per thread~\cite{guide2022cuda}. So, we set our aim at $Occupancy=12.5\%$ or $TLP=256$. %In this case, we need $ILP=4$.

% \subsection{Minimal Sufficient Parallelism: A Case Study On the STREAM Kernel}
% We consider a $a=b$ STREAM kernel~\cite{mccalpin1995stream} . This kernel is bound by the memory bandwidth. According to Little's Law, $35.93\%$ of occupancy is necessary with $ILP=1$. In $ILP=4$, we only need $10\%$ occupancy. %In this case, Section~\ref{sec:motiveOver} showed that in STREAM kernel, $Occupancy=12.5\%$ with $ILP=4$ can provide $91\%$ of the performance compared with maximal occupancy version (oversubscription) of the same implementation.

% We used 256 thread per thread blocks and ILP = 4 as building block to build STREAM Kernel. As a result, the performance of Oversubscription with such building block is $P_{Occupancy=100\%}=1291$ GB/s. On the other hand, if we reduce the occupancy to $1/8$, we get: $P_{Occupancy=12.5\%}=1172$ GB/s. The performance difference is small ($9\%$). 

% % This case study reassure that Little's Law can help figuring out the setting for the choice of building block. This case study also bring up a question: is it worthwhile to use $7/8$ for improving $9\%$ of 
% % In this simple way, we trade $9\%$ of performance for freeing $87.5\%$ of on-chip resources. 

% \subsection{Extended Building Block}\label{sec:buildingblock}
% % In the GPU, the warp is a schedule units. Program in GPU without the aware of warp might not get sufficient performance. Thus, by default, warp is a building block for GPU program. In this sense, we just extend the building block of GPU programming to a larger unit. %More specifically, we define a combination of thread-level parallel and instruction-level parallel as a programming unit, then we build implementation with this building block.

% In this research, we focus on double precision global memory access, shared memory access, and DFMA, all of which are basic of stencil computation. based on Little's Law~\cite{volkov2010better}, $ILP=4$ and $Occupancy=12.5\%$ ($TLP=256$) provides enough parallelism for all three operations. We set this as a building block for our implementation in the following research. 

% In the 2d stencil, we use ILP in the stream direction (Details refer to Section~\ref{sec:lazystreaming}).

% In 3d stencils, we compose $256\times4$ to do spatial tiling as $32\times32$. 


\color{black}

==> ___costfunction.tex <==

% \section{Performance Analysis}
% \section{Cost Function: Quantify the cost between overlapped tiling and grid level tiling}\label{sec:costfunc}

% \section{Cost Analysis: To Grid Tiling Or Not}\label{sec:costfunc}
% Interestingly, many research analyzed the overhead of synchronization~\cite{Meng:2009:PMA:1542275.1542313,zhang2019understanding,feng2010gpu}. And one of them also analyze the overhead of using global synchronization and the overhead of overlapped tiling~\cite{Meng:2009:PMA:1542275.1542313}. We also would like to analyze similar thing: to grid tiling with N.5D or to overlapped tiling with N.5D tiling. 

% Overlapped tiling suffered from overhead redundant computation, that grid tiling don't need to. But grid tiling need to pay the cost of synchronization. The former is related spacial parameters, while the later is related to temporal parameters. The analysis is not straightforward and is case to case. We divide the analysis to 2D stencil and 3D stencil in this section.
% \subsection{2D stencils}
% We use $tile_X=256$.

% Based on Equation~\ref{eqt:2doverlapped}, we have $\mathbb{V}(Overlapped)=\tfrac{256-2\times rad\times t}{256}$. Take 2d5pt as an example, we have $t=9$ and $rad=1$, So $\mathbb{V}(Overlapped)\approx93\%$

% On the other hand, for grid level tiling, based on Equation~\ref{eqt:smsize} we can go as deep as $t=15$, this is larger than the turning point, so we have: $\mathbb{L}(com)=2.05us$. Because the $\mathbb{O}(sync)=1.2us$. We have $\mathbb{V}(gridtile)\approx63\%$
% \subsection{3D stencils}
% We use $tile_X=32$ and $tile_Y=32$.

% Based on Equation~\ref{eqt:3doverlapped}, we have $\mathbb{V}(Overlapped)=\tfrac{(32-2\times rad\times t)^2}{32^2}$. Take 3d7pt as an example. We have $rad=1$. We use $t=4$, a setting also used in AN5D~\cite{DBLP:conf/cgo/MatsumuraZWEM20} and StencilGen~\cite{rawat2018domain}. So $\mathbb{V}(Overlapped)\approx56\%$. Note that in such setting, the temporal blocking is not deep enough to shift the bottleneck. 

% On the other hand, for grid level tiling, based on Equation~\ref{eqt:smsize} we can go as deep as $t=8$, this is smaller than the turning point, so we have: $\mathbb{L}(com)=2.28us$. Because the $\mathbb{O}(sync)=1.2us$. We have $\mathbb{V}(gridtile)\approx65\%>56\%\approx\mathbb{V}(Overlapped)$.

% \subsection{Summary}
% Though generally case to case, the N.5D overlapped tiling has a higher performance in low order 2D stencil, while grid N.5D tiling has higher performance in high order stencils as well as 3d stencils. 
\begin{comment}

In a high level, overlapped tiling has redundant computation, while grid level tiling has the overhead of synchronization. This section we analysis the trade off between overlapped tiling and grid level tiling. We base our analysis on 2d stencil and 3d stencil, and we use the giga-cells updated per second (GCells/s)~\cite{DBLP:conf/cgo/MatsumuraZWEM20,chen2019versatile} for performance metrics.
 % and used 2d5pt stencil and 3d7pt stencil as a case analysis

\subsection{Restrictions}


\subsection{Performance Analysis}
\subsubsection{}
 % We base the analysis of this section on the assumption that we move the bottleneck to  
% \subsubsection{2.5D stencil}
% \subsubsection{3.5D stencil}
\subsection{Cache Consumption Analysis}
\subsubsection{2.5D stencil}
 
\subsubsection{3.5D stencil}

\subsubsection{To asynchronous copy or not }

Performance model for cache usage

In this section we build performance model aim at: 

\begin{itemize}
    \item Make implementation decision. (Device-level temporal blocking or Thread Block level temporal blocking)
    \item Predict the achievable performance.
    \item Projecting necessary cache size for different design principle. 
\end{itemize}

\subsection{Dismiss halo dependencies}


In this subsection, for simplicity, we make the following assumption:
\begin{enumerate}
    \item we dismiss the dependency of halo region (find citation).
    \item we assume infinite cache size. 
\end{enumerate}

Fig~\ref{Fig:ptbexlain} shows temporal blocking implementations. As stencil is bandwidth hungry, we assume that the aim of temporal blocking is to move the bottleneck away from global memory bandwidth, and closer to shared cache bandwidth. We picture two scenarios: raw temporal blocking implementation where the shared cache space is limited. Even in this situation we can rely on over-subscription so that concurrently executable component 'magically' overlapped with each other~\cite{DBLP:conf/cgo/MatsumuraZWEM20}. We also picture a perfect temporal blocking format, relying on pipeline pattern, where computation (cache memory access) and main memory access are perfectly overlapped. We dismiss the begin and end part of the pipeline, that can be amortized. 

The analyse of raw temporal blocking is simple if it is a single thread block. Yet, practically, it relies on oversubscription for overlapping, it is hard to model the situation when the scheduler fail to do so. Those who interested in this topic can refer to previous research~\cite{DBLP:conf/cgo/MatsumuraZWEM20}. 

The following analysis is based on PTB (Perfect Temporal Blocking). The bandwidth of shared cache is $\mathbb{B}_{sc}$ and bandwidth of memory is $\mathbb{B}_{m}$. We assume that store and load to main memory using the same pipe, so that the global memory access per point is $2$. If the shared cache access time per point is $x$, and if the temporal time step is $t$. If shared memory and global memory access exactly the same amount of points, in order that bottleneck is moved from memory to shared cache, we have:

\begin{equation}
% \footnotesize
\begin{aligned}
 	\frac{x\times t}{\mathbb{B}_{sc}}\geq \frac{2}{\mathbb{B}_{gm}}
\end{aligned}\label{eqt:perfectbase}
\end{equation}

Ideally, we assume an large enough shared cache that can always saturate this requirement. Assume that the latency of synchronization is $\mathbb{T}(Sync)$, the size of the value is $\mathbb{S}(Type)$, the number of points of a single tiling is $\mathbb{D}(Tile)$. The runtime between two synchronization inside the pipeline is: 
\begin{equation}
% \footnotesize
\begin{aligned}
 	\mathbb{T}=\mathbb{T}(sync)+\frac{x\times t\times \mathbb{S}(Type)\times \mathbb{D}(Tile)}{\mathbb{B}_{sc}}
\end{aligned}
\end{equation}

Because GPU is a throughput optimized architecture, we change the aimed factor to throughput $\mathbb{THR}$, so we have:

\begin{equation}
% \footnotesize
\begin{aligned}
 	\mathbb{THR}&=\frac{\mathbb{D}(Tile)\times t}{\mathbb{T}(sync)+\frac{x\times t\times \mathbb{S}(Type)\times \mathbb{D}(Tile)}{\mathbb{B}_{sc}}}
\end{aligned}
\label{eqt:cmbottelneck}
\end{equation}
Ideally, if we have infinite cache space:
\begin{equation}
% \footnotesize
\begin{aligned}
 	\mathbb{THR}=\lim_{t \to \inf} \frac{\mathbb{B}_{sc}}{x\times \mathbb{S}(Type)}
\end{aligned}
\end{equation}
Or if the overhead of synchronization is negligible:
\begin{equation}
% \footnotesize
\begin{aligned}
 	\mathbb{THR}=\lim_{\mathbb{T}(sync) \to 0} \frac{\mathbb{B}_{sc}}{x\times \mathbb{S}(Type)}
\end{aligned}
\end{equation}

If we use Ampere A100 architecture computing 2d5pt as an example. We assume that the shared cache is its scratchpad memory. We assume that we use 256 threads per stream multiprocessor, according to Nvidia document~\cite{nvidia2019programming}, we have $\mathbb{T}(sync)=\tfrac{256}{\mathbb{THR}(sync)}=4 cycle$. Practically 2d5pt need 3 shared memory access~\cite{DBLP:conf/cgo/MatsumuraZWEM20}($x=3$).Total size of shared memory per SM is 164KB, despite implementation details, assuming half of the shared memory space is involved in the PTB, we have $\mathbb{T}(sm)=\tfrac{x\times t\times \mathbb{S}(Type)\times \mathbb{D}(Tile)}{\mathbb{B}_{sc}}=\tfrac{3\times 82 KB}{\mathbb{THR}_{sm}}=984 cycle$. This is far longer than the overhead of thread block synchronizations. Contrary, a smaller tiling as $1024\times 8 Byte$ (4 double value per thread in 256 threads) with temporal step of $1$, $\mathbb{T}(sm)=32$. The overhead of synchronization would be considerable large ($10\%$ of execution time). So the first implementation decision for PTB is:

\begin{theorem}
Consume as much shared cache as possible.
\label{the:consumecache}
\end{theorem}

\subsection{Add halo dependency}
There are three way of resolving halo dependency of a $halo=h$ stencil: 
\begin{itemize}
    \item Overlapped tiling (find citation)
    \item Wavefront synchronization to exchange information (find citation)
    \item Complex programming shape (find citation)
\end{itemize}

When halo size is small, overlapped tiling is simple with limited overhead. When halo size is large, the overhead gradually becomes unacceptable large (find citation), a complex programming shape or synchronization to exchange information in necessary. 

This subsection, we firstly analyze the performance of overlapped tiling. Then we will turn to wavefront synchronization.

\subsubsection{Overlapped tiling N.5 d tiling}

N.5D is very efficient, it reduce the overhead of halo region by one dimension. Take 2d stencil as an example, assume that the basic tiling is $Tile_x(valid)$. In order to saturate the dependency, a total of $Tile_x(load)=Tile_x(valid)+2 \times t \times h$ need to be loaded. So the valid throughput would be: 

\begin{equation}
% \footnotesize
\begin{aligned}
 	\mathbb{THR}_{2d}(valid)=\mathbb{THR}\times \frac{Tile_x(valid)}{Tile_x(load)}
\end{aligned}
\end{equation}

So the more temporal time step, the lower the valid performance. The second implementation decision for PTB is:

\begin{theorem}
\textbf{Overlapped Tiling:} choose a temporal blocking size slightly larger than the point when shared cache becomes the bottleneck.
\end{theorem}

Similarly, we can get the valid throughput for 3d stencil:

\begin{equation}
% \footnotesize
\begin{aligned}
 	\mathbb{THR}_{3d}(valid)=\mathbb{THR}\times \frac{Tile_x(valid)\times Tile_y(valid)}{Tile_x(load)\times Tile_y(load)}
\end{aligned}
\end{equation}

In 3d stencil, we have to consider one additional possibility, the overhead of overlapped tiling is too large that its overhead might be too large that surpass the advantage of temporal blocking. Would overlapped temporal blocking achieve its peak performance before the bottleneck is moved to shared memory? In this situation Equation~\ref{eqt:cmbottelneck} would become:

\begin{equation}
% \footnotesize
\begin{aligned}
 	\mathbb{THR}&=\frac{\mathbb{D}(Tile)\times t}{\mathbb{T}(sync)+\frac{2\times \mathbb{S}(Type)\times \mathbb{D}(Tile)}{\mathbb{B}_{gc}}}
\end{aligned}
\label{eqt:gmbottelneck}
\end{equation}

Similarly if the overhead of synchronization is negligible:
\begin{equation}
% \footnotesize
\begin{aligned}
 	\mathbb{THR}=\lim_{\mathbb{T}(sync) \to 0} \frac{\mathbb{B}_{gc}\times t}{2\times \mathbb{S}(Type)}
\end{aligned}
\end{equation}

We assume $Tile_x(load)=Tile_y(load)=tile$, we get:

\begin{equation}
\begin{aligned}
 	\mathbb{THR}_{3d}(valid)=\frac{\mathbb{B}_{gc}\times t}{2\times \mathbb{S}(Type)}\times \frac{tile(valid)^2}{tile(load)^2}\\
 	=\frac{\mathbb{B}_{gc}\times t}{2\times \mathbb{S}(Type)}\times \frac{(tile-2\times t\times h)^2}{tile^2}
\end{aligned}
\end{equation}

We can know from its deviation that it reaches its max when $t=\tfrac{tile}{4\times h}$. 

So, in 3d situation

\begin{lemma}
\textbf{Overlapped Tiling in 3d:} choose both the temporal blocking size slightly larger than the point when shared cache becomes the bottleneck and the size that saturate: $t=\tfrac{tile}{4\times h}$.
\end{lemma}

In order to saturate the Theorem~\ref{the:consumecache},  we increase the size of tiling, instead of increase the temporal blocking size. 

\subsubsection{Wavefront synchronization to exchange halo information}

On additional possibility is to exchange halo information. In this situation, a device-wide synchronization is necessary. We assume its overhead is $\mathbb{T}(device\_wide\_sync)$. 

\begin{equation}
% \footnotesize
\begin{aligned}
 	\mathbb{THR}(valid)=\frac{Tile}{\frac{Tile}{\mathbb{THR}}+\mathbb{T}(device\_wide\_sync)}
\end{aligned}
\end{equation}

Additionally, apart from the amortized portion, assume that the halo region has a size of $\mathbb{HALO}$ the Equation~\ref{eqt:perfectbase} is changed to the following format:

\begin{equation}
% \footnotesize
\begin{aligned}
 	\frac{x\times t\times{Tile}}{\mathbb{B}_{sc}}\geq \frac{2\times t \times{\mathbb{HALO}}+2\times{Tile}}{\mathbb{B}_{gm}}
\end{aligned}\label{eqt:wvflimit}
\end{equation}

 
 \begin{theorem}
\textbf{Wavefront synchronization method:} choose a tiling size slightly larger than the point when Equation~\ref{eqt:wvflimit} is saturated.
\end{theorem}

Heuristically, we assume that temporal blocking is large enough so that we can simplify the requirement:

\begin{equation}
% \footnotesize
\begin{aligned}
 	\frac{x\times{Tile}}{\mathbb{B}_{sc}}\geq \frac{2\times{\mathbb{HALO}}}{\mathbb{B}_{gm}}
\end{aligned}\label{eqt:wvflimit}
\end{equation}

In order to saturate the Theorem~\ref{the:consumecache}, we increase the temporal blocking size, instead of increase the tiling size. 

\subsubsection{Complex programming shape}
 We dismiss complex programming shape because:
 \begin{itemize}
     \item When halo is low, its overhead of overlapped tiling is low
     \item Complex shape is not memory alignment friendly, which make it hard to achieve theoretical performance. (find citation) 
 \end{itemize}

\subsection{Choose tiling size based on concurrency analysis}
 
\subsection{Add the scale of cache}

\begin{itemize}
    \item Minimal cache size for perfect temporal blocking
    \item Predict performance based on A100 cache size
    \item Predict performance when cache size keep increasing.
\end{itemize}
In this section, we analysis the minimal shared cache size that required for achieving perfect temporal blocking. And the different cache requirement for overlapped tiling and wavefront synchronization. Then based on A100, we give an analysis of its


% This subsection use A100 as an example. The cache size is 164 KB. We assume 2d stencil has a tile of $256\times y$, while 3d stencil has a tile of $32\times 32\times z$ for programmable practice. 

%  1.2. when halo is large, it could is not significant outperform wavefront synchronization in theory (will discuss this in details). 

\end{comment}

==> ___introduction_gpuorient.tex <==
\section{Introduction}

General Purpose Graphics Processing Units (GPGPUs) support over $34.2\%$ of the top HPC system~\cite{top500}. %Over the last decade, GPGPUs power many High Performance Applications~\cite{selvitopi2022extreme,zvyagin2022genslms,kurth2018exascale} and many Deep Learning Training Platforms~\cite{dillon2017tensorflow, paszke2019pytorch}. A study in programming principle that improve performance can benefit a wide range of systems, platforms and applications. 
When observing the latest GPUs\footnote{We focus on Nvidia GPUs in this paper since the continuity of GPU products by Nvidia over decades provides the grounds for analyzing the evolution in GPUs.}, there are notable changes in key characteristics. We can observe a significant drop in instruction latency. Take double precision floating point multiply and add instruction (DFMA), as an example. {The latency of DFMA dropped from 48 cycle in K80~\cite{wong2010demystifying} to 4 cycle in A100~\cite{abdelkhalik2022demystifying}.} Although GPU is considered a throughput-optimized platform, while CPU is considered a latency-optimized platform, the GPU vendor also optimized the latency in GPU. And these drops in latency make it easier to achieve desirable performance and tolerate lower occupancy, i.e., easier to hide latency.\wahib{@Lingqi: this example is not complete. You should say something along the lines of how this reduction in DFMA leads to fewer threads, for example, by reporting how many threads a call to a gemm API in cublas need now vs. in old generations.} 

Another observation is a significant increase in cache capacity. For example, the total capacity of the user-managed cache (shared memory) increased from $720$ KB in K20~\cite{kepler} to $17712$ KB in A100~\cite{nvidiaa100}. Additionally, the capacity of the L2 cache has increased from $1.5$ MB in K20~\cite{kepler} to $40$ MB in A100~\cite{nvidiaa100}. Therefore, the shared memory capacity has increased $24.6$x and the L2 cache capacity has increased $26.7$x over the last decades. 

In addition, GPUs are providing features that are supported by CPUs for years. Examples include dynamic programming, cooperative groups, and hardware pre-fetch (shared memory asynchronous copy)~\cite{guide2022cuda}. 

Unfortunately, we observed very limited change in the GPU programming model and execution model, i.e., maximize parallel execution~\cite{guide2022cuda} and offload execution. 

Stencils are common computational patterns that exist widely in many scientific applications. Temporal blocking is a widely used optimization in iterative stencil optimization~\cite{maruyama2011physis,malas2015multicore,endo2018applying,wellein2009efficient}. The key of temporal blocking is to execute a batch of time steps as a whole to get the benefit of the data temporal locality. Temporal blocking resolves dependency between time steps either by overlapped tiling~\cite{DBLP:conf/cgo/MatsumuraZWEM20,rawat2018domain,10.1145/2304576.2304619,Meng:2009:PMA:1542275.1542313} or by complicated geometry (e.g. diamond~\cite{bondhugula2017diamond} and hexagonal tiling~\cite{grosser2014hybrid,grosser2014relation}). Either way, temporal blocking increases the data dependency as the temporal blocking size increases (the time steps inside a tiling) and gradually changes the kernel from throughput bound to latency bound. Additionally, the long dependency between registers might also influence performance~\cite{DBLP:conf/cgo/MatsumuraZWEM20} in the deep temporal blocking algorithm.

In this research, we choose the latest GPU platform, A100. We focus on the programming model part and ask a very simple question:{ can we kick off the "maximize parallel execution" principle in GPU programming? }. We summarized two programming principle: 1. Kick off oversubscription, i.e. get sufficient concurrency with minimal building block, and then use the on-chip resources released for aggressive optimization. 2. Kick off massive parallelism, and embrace grid-level tiling. We then propose several optimizations that derived from these principles. We use these optimizations to optmize temporal blocking kernel and propose EBISU. With the released on-chip resources we proposed dependency free streaming method. As a result we achieve ... in speedup in 2d stencils compared with the best state of the art temporal blocking implementations. Additionally, we used grid level tiling and resolve inter thread block depdendency by grid level synchronization. As a result in 3d stencils compared with the best state of the art temporal blocking implementations.
% In this paper, we 


Contribution of this paper includes the following.

\begin{itemize}
    % \item We benchmark the Nvidia GPU Lineage. We summarize the findings and proposed design principles to solve the performance issue in the state-of-the-arts temporal blocking implementations.
    \item We analyse the GPU programming principle and propose two principles to replace the "maximize parallel execution principle", i.e. minimal concurrency and minimal workload per grid. 
    \item We used the two principle to design two temporal blocking implementation in GPU, i.e. dependency free streaming and grid-level temporal blocking
    \item We include a performance analysis for implementation decision and analyze the desired scratchpad memory for the implementation.
    % design principle to solve the limitation in the state-of-the-arts implementation of GPU temporal blocking algorithm.
    \item Our implementation achieve significant speedup over the state of the state of the art implementation. We will open source if the paper get accepted. 
\end{itemize}

==> ___programmingguide_NOTINUSE.tex <==
\section{GPU Programming: Principle, its Myths and Kicking It Away}

We summarize two principles of GPU programming: Oversubscription and Massive Parallelism. GPU consists of large amounts of processing unit, so it is intuitive to launch as many threads, or thread blocks, as possible to express parallelism (Oversubscription, or Massive Parallelism). In order to do this, the workload should also be as large as possible such that the workload itself can offer enough parallelism (Massive Execution). In the GPU programming guide~\cite{guide2022cuda}, Oversubscription and Massive Execution are summarized as Maximize Parallel Execution.
% Also, GPU used single-thread multiple-data (STMD) programming model, so regular behavior between STMD unit (a warp) is prerequisite for best performance. 

% In this research, we mainly focus on the Oversubscription and Massive Parallelism principle (Maximize parallel execution in CUDA Programming guide~\cite{guide2022cuda}). 

% \todo{find citation}
\subsection{Kick Oversubscription (Max Parallelism) away}\label{sec:motiveOver}
\subsubsection{Overview of Oversubscription}
Generally, oversubscription means that the execution of thread blocks larger than the hardware limit, then the dynamic scheduler is leveraged for workload assignment. This method automatically achieves the maximum occupancy that the device can support. So, this principle involves two assumptions: 1. dynamic scheduler always performs well; and 2. highest available occupancy always benefits performance. However, many by-passsing schedulers~\cite{aila2009understanding,chen2010dynamic,ma2020rammer} shows that dynamic scheduler not always outperform manual efforts. Furthermore, Volkov~\cite{volkov2010better} shows that low occupancy might outperform higher occupancy with the help of Instruction Level Parallelism (ILP). Additionally, ILP is now summarized as a principle in the CUDA programming guide~\cite{guide2022cuda} now. 

\textbf{However, existing researches, including Volkov's research~\cite{volkov2010better}, are still chasing the maximal available occupancy hardware can provide.} In this research, we extend the definition of Oversubscription as: \textbf{Oversubscription happended when launched thread blocks exceed the concurrency provided by the hardware.} Because the thread blocks launched, even thought concurrently reside in the hardware, might not use resources efficiently when Oversubscription happened.% and suffer from Diminishing Marginal Returns.

\subsubsection{It is all about concurrency!}
The analysis of the following section is an extension of Volkov's research~\cite{volkov2010better}. We based on our analysis on Little's Law too. Little's Law use Latency $\mathbb{L}$ and Throughput $\mathbb{THR}$ to infer the concurrency $\mathbb{C}$ of the given hardware:
\begin{equation}
     \mathbb{C}=\mathbb{L}\times\mathbb{THR}
\end{equation}

$\mathbb{L}$ of an instruction can be gathered by microbenchmarks.~\cite{wong2010demystifying}. $\mathbb{THR}$ of an instruction can refer to nvidia documents~\cite{guide2022cuda,nvidiaa100}.

As long as the Parallelism $\mathbb{P}$ provided by the software is larger than the concurrency provided by the hardware, we consider that the software saturate the hardware:

\begin{equation}
     \mathbb{P}\ge\mathbb{C}
\end{equation}

There are two ways of providing Parallelism: Thread Level Parallelism (TLP) and Instruction Level Parallelism (ILP), according to Volkov's research. We consider:

\begin{equation}
     \mathbb{P}={TLP}\times{ILP}
\end{equation}

We need to find any combination of TLP and ILP that saturates:

\begin{equation}
     {TLP}\times{ILP}\ge\mathbb{C}=\mathbb{L}\times\mathbb{THR}
\end{equation}

Occupancy is usually considered a representation of Parallelism. But it is only true when the program only rely on TLP for Parallelism. Basically, $Occupancy=12.5\%$ when $TLP=256$. In this case, if $ILP=1$, then $\mathbb{P}=256$.

\subsubsection{Get performance in low occupancy} 
To maintain a certain level of parallelism, we can reduce occupancy (TLP) and increase (ILP) in the same time. We reduce the occupancy to a point that it wont increase the resources per thread blocks. In the current hardware (A100), further reduce occupancy to less than $12.5\%$ won't increase the available register per thread~\cite{guide2022cuda}. So, we set our aim at $Occupancy=12.5\%$ or $TLP=256$. In this case we need $ILP=4$ 

To illustrate it, we consider a STREAM kernel. STREAM kernel is bound by memory bandwidth. According to Little's Law, $35.93\%$ of occupancy is necessary with $ILP=1$. In $ILP=4$, we only need $10\%$ of occupancy. %In this case, Section~\ref{sec:motiveOver} showed that in STREAM kernel, $Occupancy=12.5\%$ with $ILP=4$ can provide $91\%$ of the performance compared with maximal occupancy version (oversubscription) of the same implementation.

To further illustrate this idea, we use a $a(i)=b(i)$ STREAM kernel~\cite{mccalpin1995stream} in A100 as an example. We use 256 thread per thread blocks and ILP = 4. As a result, the performance $P$ of Oversubscription is $P_{Oversubscription}=1291$ GB/s. On the other hand, if we reduce the occupancy to $1/8$, we get: $P_{Occupancy=12.5\%}=1172$ GB/s. In this simple way, we trade $9\%$ of performance for freeing $87.5\%$ of on-chip resources. 

\subsubsection{Extended Building Block}\label{sec:buildingblock}
In GPU, warp is a schedule units. Program in GPU without the aware of warp might not get sufficient performance. So warp is a building block for GPU program. In this sense, we extend the building block to a unit that saturate the device. More specifically, we define a combination of thread level parallel and instruction level parallel as a programming unit, then we build implementation with this building block. \textbf{Because the building block itself has already saturate the device, any implementation built from the building block can provide enough concurrency to saturate the device}. 

In this research we consider double precision global memory access, shared memory access and DFMA, all of which are basic of stencil computation. based on Little's Law~\cite{volkov2010better}, ILP=4 and Occupancy=12.5\%(TLP=256) provides enough parallelism for all three operations. We set this as a building block for our implementation for the following research. In 2d stencil, we use ILP in the stream direction (Details refer to Section~). In 3d stencils, we compose $256\times4$ to do spacial tiling as $32^2$. 

\begin{comment}
\subsubsection{Asynchronous Shared Memory Copy}
The new asynchronous shared memory copy A100~\cite{nvidiaa100} also reduce the requirement of high occupancy. To illustrate it, with asynchronous copy, we are able to overlap the memory access with computation without blocking. Otherwise, a minimal of 2 thread blocks per stream multiprocessor is necessary to hide memory access latency. Additional thread blocks increase the overhead if grid synchronization~\cite{zhang2020study,dalmia2022improving} and reduce the maximal tiling size per thread block. 
\end{comment}

\subsection{Kick Massive Execution away}
\begin{figure}[t]
\centering
 \includegraphics[width=0.47\textwidth]{FIG/BandwidthvsSize.pdf}
 \caption{$a(i)=b(i)$ STREAM benchmark~\cite{mccalpin1995stream}, repeat 1000 times in A100 (theory bandwidth=$1555$ GB/s), the relationship between the total domain size and the bandwidth achieved. The device achieved 86\% of peak performance in 54 MB ($0.1\%$ of the device memory size (40GB) in A100)}
 \label{fig:bandvssize}
\end{figure}
\input{TABLE/KernelOverhead.tex}

\subsubsection{Overview of Massive Execution}
GPUs are suitable for massive parallelism. So instinctively people pushes massively available workloads to GPU. This principle works in most situations and existing research focuses mainly on the domain size as large as possible ~\cite{chen2019versatile,DBLP:conf/cgo/MatsumuraZWEM20,rawat2018domain} without questioning how large is enough. To the best of our knowledge, the research conducted by Eberius et al.~\cite{saturationGPU} was the first to ask this question.
\subsubsection{Minimal sufficient workload}
We only need minimal sufficient workload for a given algorithm in a given device. As an example, we use the same kernel in Section~\ref{sec:motiveOver}. We gradually increase the size of the domain and record the performance. As Figure~\ref{fig:bandvssize} shows, this kernel can achieve $86\%$ of practical peak performance with the size of the $54MB$ domain. And in 27MB it can even benefit from L2 cache.  

% \textbf{The knowledge here is: we can tile the domain that for each tiling the device is able to get sufficient parallelism, while small enough to get the benefit from cache locality.}

Now that smaller amount of parallelism can saturate the device. Why not using minimal necessary workload that can fit into the cache system, while large enough to saturate the device? 

%Empirically, we need to pay the cost of kernel overhead, but get the benefit of reside data in cache. The ability to better use cache system with smaller workload is known as super linear speedup in HPC.~\cite{ristov2016superlinear}. As an additional step, now that on-chip resources are so large, why not use grid synchronization to replace kernel launch, so that we are able to use the on-chip resources more effectively?

\subsubsection{The Cost We Pay}
One of the reason for Massive Execution is we need to amortize the overhead of kernel overhead~\cite{zhang2019understanding,zhang2020study}. Intuitively, if the workload is not enough to ensure that a kernel lasts long enough, the proportion of kernel overhead would be significant. Many efforts when into kernel fusions~\cite{DBLP:conf/sc/WahibM14,DBLP:conf/ics/GysiGH15} to solve such issues. To quantify the overhead, we followed the research of Zhang et al.~\cite{zhang2020study}, we adjust their code for A100 and report the kernel overhead in Table~\ref{tab:overhead}. We also report the grid synchronization overhead because it can be an alternative for kernel launch overhead, as Table~\ref{tab:overhead} shows.% Additionally, 


\subsubsection{The Benefit We Gain}
The main benefit of kicking off massive parallelism and adjusting to minimal parallelism is the better cache locality as can be conveyed from Figure~\ref{fig:bandvssize}. Apart from the $40$ MB large L2 cache in A100.% , by not obeying the principle of massive parallelism. The detail analysis of the trade off is case to case. 

\subsubsection{A Step Forward: On-Chip Resources.} We can also get benefit from the on-chip resources, including 17.30 MB of shared memory and 27 MB of register files. These large amount resources would be wipe out in between kernel launch. We can aggressively fuse the kernel and use grid level synchronization to handle unavoidable inter thread block dependency. It is hard to quantify the benefit of using grid synchronization in this manner. However, we can analyze this question in an opposite anger: what is the cost of wipe out this large amount of on-chip resources? Take the 17.3MB of shared memory in A100 as an example. With $1555$ GB/s global memory bandwidth, we need about $12$ us to fill data into shared memory. If we repeatedly load this amount of data to on-chip while not keep the reusable data, we pay the cost of $12$ us upon each loading. Note that this overhead is about an order of magnitude larger than the kernel launch overhead as Table~\ref{tab:overhead} shows. 


\subsection{Benefit of kicking GPU programming principles away} 
We anticipate that kicking oversubscription free large amounts of on-chip resources. These freed resources can automatically benefit algorithms that suffer from \textbf{register pressure}~\cite{DBLP:conf/cgo/MatsumuraZWEM20,Rawat:2018:ROS:3200691.3178500,stock2014framework} or that are \textbf{cache capacity 
starving}~\cite{maruyama2014optimizing,8820786,wellein2009efficient}. Additionally, smaller amounts of concurrently running threads reduce contention; thus \textbf{reduce overhead of synchronization}~\cite{guide2022cuda,zhang2020study,dalmia2022improving}. 

Also, using minimal sufficient execution make the implementation \textbf{cache locality friendly}. 


% Small enough workload to saturate the device
% -> Grid level tiling. 
% Small benchmark to support.

% \subsection{Highlights that Motivates This Research}
% This section, we revisit general GPU Programming Principles, i.e. Oversubscription and Massive Execution. This research don't argue against these principles. However, by simply kicking off these principles, programmers can get alternative chances to optimize their programs. We summarize the benefits of doing so as follow: 
% \begin{itemize}
%     \item Alleviate register pressure
%     \item Support cache capacity starving algorithm
%     \item Reduce overhead of synchronization
%     \item Better cache locality
% \end{itemize}

% , support cache capacity starving algorithm, reduce overhead of synchronization and better cache locality.

% suffer from Diminishing Marginal Returns.

==> ___proposal.tex <==
\section{Kick of the GPU Programming Principle}
% \todo{merge to the previous section}
We proposed two principles to get rid of the "Massive Parallel Execution" principle in GPU programming. We base our discussion on the Nvidia A100 GPU. However the analysis can be generalized to any other platforms.

\subsection{Principle 1: Minimal necessary occupancy (Kick off Oversubscription)}
% \subsubsection{$\mathbf{Occupancy}=\mathbf{12.5\%}$ is what we need}
\subsubsection{It is all about concurrency!}
The analysis of this section is an extension of Volkov's research~\cite{volkov2010better}. We based on our analysis on Little's Law. Little's Law use Latency $\mathbb{L}$ and Throughput $\mathbb{THR}$ to get concurrency $\mathbb{C}$, the maximal concurrency provided by the hardware:
\begin{equation}
     \mathbb{C}=\mathbb{L}\times\mathbb{THR}
\end{equation}

$\mathbb{L}$ of an instruction can be gathered by microbenchmarks.~\cite{wong2010demystifying}. $\mathbb{THR}$ of an instruction can refer to nvidia documents~\cite{guide2022cuda,nvidiaa100}.

As long as the Parallelism $\mathbb{P}$ provided by the software is larger than the concurrency provided by the hardware, we consider that the software saturate the hardware:

\begin{equation}
     \mathbb{P}\ge\mathbb{C}
\end{equation}

There are two ways of providing Parallelism: Thread Level Parallelism (TLP) and Instruction Level Parallelism (ILP), according to Volkov's research. We consider:

\begin{equation}
     \mathbb{P}={TLP}\times{ILP}
\end{equation}

We need to find any combination of TLP and ILP that saturates:

\begin{equation}
     {TLP}\times{ILP}\ge\mathbb{C}=\mathbb{L}\times\mathbb{THR}
\end{equation}

Occupancy is usually considered a representation of Parallelism. But it is only true when the program only rely on TLP for Parallelism. Basically, $Occupancy=12.5\%$ when $TLP=256$. In this case, if $ILP=1$, then $\mathbb{P}=256$.

\subsubsection{Get performance in low occupancy} 
To maintain a certain level of parallelism, we can reduce occupancy (TLP) and increase (ILP) in the same time. We reduce the occupancy to a point that it wont increase the resources per thread blocks. In the current hardware (A100), further reduce occupancy to less than $12.5\%$ won't increase the available register per thread~\cite{guide2022cuda}. So, we set our aim at $Occupancy=12.5\%$ or $TLP=256$. In this case we need $ILP=4$ 

To illustrate it, we consider a STREAM kernel. STREAM kernel is bound by memory bandwidth. According to Little's Law, $35.93\%$ of occupancy is necessary with $ILP=1$. In $ILP=4$, we only need $10\%$ of occupancy. In this case, Section~\ref{sec:motiveOver} showed that in STREAM kernel, $Occupancy=12.5\%$ with $ILP=4$ can provide $91\%$ of the performance compared with maximal occupancy version (oversubscription) of the same implementation.


% To answer the question, we consider three conditions: compute bound, shared memory bandwidth bound and global memory bound.

% We use microbenchmark provided by Wong et al.~\cite{wong2010demystifying} to collect hardware data. Due to the space limit, we only provide the summary of the results in this section. 

% If the kernel is compute bound and DFMA (double precision multiply and add instruction) instruction mainly bound the performance, according to Little's Law, $6.25\%$ of occupancy is necessary without relying on instruction level parallelism ($ILP=1$). 

% If the kernel bound by memory bandwidth, according to Little's Law, $35.93\%$ of occupancy is necessary with $ILP=1$. We can rely on $ILP$ to reduce the necessary occupancy. With $ILP=4$, the necessary occupancy is reduced to $10\%$. STREAM kernel is a memory bandwidth bound kernel. Section~\ref{sec:motiveOver} showed that in STREAM kernel, $Occupancy=12.5\%$ can provide good enough performance with $ILP=4$. 

% If the kernel is bound by shared memory bandwidth, according to Little's Law, $18.75\%$ of occupancy is necessary without relying on instruction level parallelism (ILP). So, we with $ILP=4$. we can reduce the necessary occupancy to $4.68\%$.



\subsubsection{Extended Building Block}
In GPU, warp is a schedule units. Program in GPU without the aware of warp might not get sufficient performance. So warp is a building block for GPU program. In this sense, we extend the building block to a unit that saturate the device. More specifically, we define a combination of thread level parallel and instruction level parallel as a programming unit, then we build implementation with this building block. \textbf{Because the building block itself has already saturate the device, any implementation built from the building block can provide enough concurrency to saturate the device}. 

In this research we consider double precision global memory access, shared memory access and DFMA, all of which are basic of stencil computation. based on Little's Law~\cite{volkov2010better}, ILP=4 and Occupancy=12.5\% provides enough parallelism for all three operations. We set this as a building block for our implementation for the following research. 
\subsubsection{Asynchronous Shared Memory Copy}
The new asynchronous shared memory copy A100~\cite{nvidiaa100} also reduce the requirement of high occupancy. To illustrate it, with asynchronous copy, we are able to overlap the memory access with computation without blocking. Otherwise, a minimal of 2 thread blocks per stream multiprocessor is necessary to hide memory access latency. Additional thread blocks increase the overhead if grid synchronization~\cite{zhang2020study,dalmia2022improving} and reduce the maximal tiling size per thread block. 


\subsection{Principle 2: Minimal Necessary Workloads each time (Kick off Massive Execution)}
\input{TABLE/KernelOverhead.tex}
Now that smaller amount of parallelism can saturate the device. Why not using minimal necessary workload that can fit into the cache system, while large enough to saturate the device? Empirically, we need to pay the cost of kernel overhead, but get the benefit of reside data in cache. The ability to better use cache system with smaller workload is known as super linear speedup in HPC.~\cite{ristov2016superlinear}. As an additional step, now that on-chip resources are so large, why not use grid synchronization to replace kernel launch, so that we are able to use the on-chip resources more effectively?

\subsubsection{The Cost We Pay}
One of the reason for Massive Execution is we need to amortize the overhead of kernel overhead~\cite{zhang2019understanding,zhang2020study}. Intuitively, if the workload is not enough to ensure that a kernel lasts long enough, the proportion of kernel overhead would be significant. Many efforts when into kernel fusions~\cite{DBLP:conf/sc/WahibM14,DBLP:conf/ics/GysiGH15} to solve such issues. To quantify the overhead, we followed the research of Zhang et al.~\cite{zhang2020study}, we adjust their code for A100 and report the kernel overhead in Table~\ref{tab:overhead}. We also report the grid synchronization overhead because it can be an alternative for kernel launch overhead, as Table~\ref{tab:overhead} shows.% Additionally, 


\subsubsection{The Benefit We Gain}
The main benefit of kicking off massive parallelism and adjusting to minimal parallelism is the better cache locality as can be conveyed from Figure~\ref{fig:bandvssize}. Apart from the $40$ MB large L2 cache in A100, we can also get benefit from the on-chip resources, including 17.30 MB of shared memory and 27 MB of register files, by not obeying the principle of massive parallelism. The detail analysis of the trade off is case to case. 
\subsubsection{The cost of wipe out on-chip resources}
It is hard to quantify the benefit of using on-chip resources. But we can analyze it in an opposite anger: what is the cost of wipe out this large amount of on-chip resources? Take the 17.3MB of shared memory in A100 as an example. With $1555$ GB/s global memory bandwidth, we need about $12$ us to fill data into shared memory. If we repeatedly load this amount of data to on-chip while not keep the reusable data, we pay the cost of $12$ us upon each loading. However, these data would be unavoidably wiped out if one kernel finish execution. Note that this overhead is far large than the kernel launch overhead as Table~\ref{tab:overhead} shows. 

% \subsubsection{Grid Level Tiling with Grid Synchronization}
% We propose to add a grid level tiling on above of the thread block level tiling. And add a grid level synchronization to handle the dependency between thread blocks. Though hard to determine the tiling size, we simply define a greedy principle for grid level tiling: \textbf{tile the domain such that the whole tiling can fit into the scratchpad memory.} We will discuss the trade off of using grid tiling in temporal blocking in Section~\ref{sec:costfunc}. 

\subsection{Summarize}
This section proposed minimal necessary occupancy and minimal necessary workload principles. Note that these principles do not directly optimize the performance of any given application. However, these principles give opportunities for new aggressive optimizations. In the following two sections, we will discuss aggressive optimizations for stencils that built on top of these 
two principles. 

